Stretching Sentence-pair NLI Models to Reason over Long Documents and Clusters

Natural Language Inference (NLI) has been extensively studied by the NLP community as a framework for estimating the semantic relation between sentence pairs. While early work identified certain biases in NLI models, recent advancements in modeling and datasets demonstrated promising performance. In this work, we further explore the direct zero-shot applicability of NLI models to real applications, beyond the sentence-pair setting they were trained on. First, we analyze the robustness of these models to longer and out-of-domain inputs. Then, we develop new aggregation methods to allow operating over full documents, reaching state-of-the-art performance on the ContractNLI dataset. Interestingly, we find NLI scores to provide strong retrieval signals, leading to more relevant evidence extractions compared to common similarity-based methods. Finally, we go further and investigate whole document clusters to identify both discrepancies and consensus among sources. In a test case, we find real inconsistencies between Wikipedia pages in different languages about the same topic.

==> Cluster NLI paper - revised/macros.tex <==
% \usepackage[notes=true, done=false, later=true, ]{dtrt}

% \newcommand{\tal}[1]{\dtcolornote[Tal]{blue}{#1}}
% \newcommand{\sihao}[1]{\dtcolornote[Sihao]{orange}{#1}}
% \newcommand{\alex}[1]{\dtcolornote[Alex]{red}{#1}}
% \newcommand{\senaka}[1]{\dtcolornote[Senaka]{purple}{#1}}


\newcommand{\STAB}[1]{\begin{tabular}{@{}c@{}}#1\end{tabular}} % For rotating text in tables

% \newtheorem{theorem}{Theorem}
% \numberwithin{theorem}{section}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{observation}[theorem]{Observation}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{claim}[theorem]{Claim}

% \theoremstyle{definition}
% \newtheorem{definition}[theorem]{Definition}
%\theoremstyle{remark}
% \newtheorem{remark}[theorem]{Remark}
% \newtheorem{assumption}[theorem]{Assumption}
% \newenvironment{proofsketch}{\noindent{\bf Proof Sketch}\hspace*{1em}}{\qed\bigskip}

%%% Algorithm %%%
% \newcommand*\Funct[2]{\textsc{#1}(#2)}
% \newcommand*\Let[2]{\State #1 $\gets$ #2}
% \renewcommand{\Comment}[2][.44\linewidth]{%
%   \leavevmode\hfill\makebox[#1][l]{{\tiny $\triangleright$}~#2}}
% \algrenewcommand\algorithmicindent{1.0em}%

\floatname{algorithm}{Algorithm}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
%%%%%%%%%%%

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\indep}{\perp \!\!\! \perp}
\DeclareMathOperator{\softmax}{Softmax}
\newcommand{\prob}[1]{\mathbb{P}\left( {#1} \right)}

\newcommand{\newpar}[1]{\noindent\textbf{{#1}~}}
% \newcommand{\newpar}[1]{\paragraph{#1}}

%%% NLI %%%
% \newcommand{\ourmodel}{\textit{se}N\textit{t}LI\xspace}
\newcommand{\ourmodel}{\textsc{seNtLI}\xspace}
\newcommand{\prem}{X_{\mathrm{prem}}}
\newcommand{\hyp}{X_{\mathrm{hyp}}}
% \newcommand{\prem}{x_{\mathrm{prem}}}
% \newcommand{\hyp}{x_{\mathrm{hyp}}}
\newcommand{\func}{f}
\newcommand{\summac}{\textsc{SummaC}\xspace}
%%%%%%%%%%%





% \titlespacing*{\subsection}{0pt}{.35\baselineskip}{.25\baselineskip}
% \titlespacing*{\subsubsection}{0pt}{.35\baselineskip}{.25\baselineskip}
% \titlespacing*{\section}{0pt}{.35\baselineskip}{.25\baselineskip}
% \renewcommand{\paragraph}[1]{\vspace{0.2cm}\noindent\textbf{#1}}
\newcommand{\parhead}[1]{\noindent\textbf{#1}}

% \newcommand{\tpf}[1]{\noindent\textbf{#1.}}
% %\definecolor{darkgreen}{rgb}{0.0, 0.2, 0.13}
% \definecolor{darkgreen}{rgb}{0.31, 0.47, 0.26}
% \definecolor{Gray}{gray}{0.95}
% \makeatletter
% \renewcommand{\paragraph}{%
%   \@startsection{paragraph}{4}%
%   {\z@}{0.75ex \@plus 1ex \@minus .2ex}{-1em}%
%   {\normalfont\normalsize\bfseries}%
% }
% \makeatother

==> Cluster NLI paper - revised/sections/app_binary.tex <==
\section{Zero-shot binary classification}\label{sec:binary_aggr}

DocNLI uses only two classes, ``entail'' vs.\ ``not entail'', by merging the ``neutral'' and ``contradiction'' definitions. 
The ``not entail'' instances are created with both rule-based and LM-based local perturbations over the positive pairs. This results in a slightly different task definition than NLI since even altered (i.e., ``fake'') texts can still factually agree with the hypothesis~\citep{schuster-etal-2020-limitations}. \citet{yin-etal-2021-docnli} account for this by augmenting the training set, but zero-shot NLI models might be affected by this provenance-based rather than factual-based partition of the test set.


Since NLI models are commonly trained with three target labels, adjusting to a two-way classification requires some modifications. Being a zero-shot setting, we cannot train the model's internal representations to adjust to this new label space. Instead, we can define an aggregation method. We experiment with the following variants:
\begin{enumerate}[leftmargin=*]
    \item \textbf{Entailment threshold}:  predicting ``entail'' if $p_e > T$, else ``not entail''.
    \item \textbf{Contradiction threshold}:  predicting ``not entail'' if $p_c > T$, else ``entail''.
    \item \textbf{Binary softmax}:  recompute the softmax without $s_n$, and predict ``entail'' if $\softmax(s_e, s_c)[e] > T$, else ``not entail''. 
\end{enumerate}
$T$ is a decision threshold that we can either set to some arbitrary value such as $0.5$, or calibrate it on a small set of labeled data. 



Table~\ref{tab:docnli_2_aggr} presents the performance of the three aggregation methods with or without tuning $T$ on 500 random examples for the development set (with $0.05$ intervals). Thresholding on $p_e$ performs best and gives higher precision compared to the binary softmax that discards the 'neutral' score. \
Yet, all three options perform well, with different trade-offs between precision and recall, motivating the use of simple heuristics in the absence of supervised data for the target task. In the following experiments, we use the 'e' threshold method.
Tuning $T$ significantly improves the $F_1$ score by sacrificing recall for precision. We find the optimal threshold to be $0.95$, meaning that we predict 'entail' only when the model is highly confident in this relation.


\begin{table*}[t]
    \centering
    \small
    \resizebox{0.85\linewidth}{!}{
    \begin{tabular}{lc|ccc|ccc|ccc}
    \toprule
    \multicolumn{2}{c}{}& \multicolumn{3}{c}{\underline{0.2\% of DocNLI Dev.}} & \multicolumn{3}{c}{\underline{DocNLI Dev.}} & \multicolumn{3}{c}{\underline{DocNLI Test}} \\
    % \cmidrule{3-5} \cmidrule{7-8} 
    Aggregation & \multicolumn{1}{c}{$T$} & \multicolumn{1}{c}{Prec.} &  \multicolumn{1}{c}{Recall} &  \multicolumn{1}{c}{$F_1$(E)} & \multicolumn{1}{c}{Prec.} &  \multicolumn{1}{c}{Recall} &  \multicolumn{1}{c}{$F_1$(E)} & \multicolumn{1}{c}{Prec.} &  \multicolumn{1}{c}{Recall} &  \multicolumn{1}{c}{$F_1$(E)}\\
    \midrule
        'e' threshold & 0.5 & .198 & .746 & .313 & .216 & .810 & .341 & .220 & .800 & .345\\
                    & tuned & .319 & .610 & .\textbf{419} & .312 & .594 & .\textbf{409} & .313 & .589 & .\textbf{408}\\
        \midrule
        'c' threshold & 0.5 & .187 & .966 & .313 & .182 & .969 & .306 & .182 & .969 & .306 \\
                    & tuned & .244 & .915 & .386 & .230 & .872 & .364 & .230 & .872 & .364\\
        \midrule
        bin.\ softmax & 0.5 & .195 & .966 & .324 & .192 & .949 & .319& .193 & .949 & .321\\
            & tuned & .273 & .847 & .413 & .263 & .806 & .397 & .263 & .807 & .397 \\
                    
        \bottomrule
    \end{tabular}
    }%
    \caption{Different aggregation methods for converting predictions of a three-way NLI model to a binary label space. Aggregating by the score of the entailment class performs best. Tuning the threshold on random 500 examples (0.2\% of full Dev.) further improves the precision and $F_1$ scores, compared to the naive $0.5$ baseline.}
    \label{tab:docnli_2_aggr}
\end{table*}

==> Cluster NLI paper - revised/sections/app_dataset.tex <==
\section{\summac Evaluation}\label{app:summac}

\begin{table*}[t]
\small
    \centering
    % \resizebox{1.05\linewidth}{!}{
    % \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l|dddddd|d}
    \toprule
    Method & \multicolumn{1}{c}{CGS} & \multicolumn{1}{c}{XSF} & \multicolumn{1}{c}{poly}& \multicolumn{1}{c}{factC} & \multicolumn{1}{c}{sumEv}& \multicolumn{1}{c}{frank} & \multicolumn{1}{c}{AVG}\\
    % \cmidrule{2-4}
    \midrule
    $\summac_{\mathrm{ZS}}$ & 70.4 & 58.4 & \textbf{62}.\textbf{0} & 83.8 & 78.7 & 79.0 & 72.1 \\
    \midrule
    \ourmodel  (soft) & 79.3 & 59.3 & 52.4 & \textbf{89}.\textbf{5} & 77.2 & \textbf{82}.\textbf{1} & 73.3 \\
    + Rerank (soft) & 79.6 & 62.7 & 52.8 & 86.1 & 78.5 & 80.4 & 73.3 \\
    + Rerank (hard)  & \textbf{80}.\textbf{5} & \textbf{64}.\textbf{2} & 55.1 & 83.3 & \textbf{79}.\textbf{7} & 78.4 & \textbf{73}.\textbf{5} \\ 
     \bottomrule
    \end{tabular}
        % }%
    % \vspace{-5pt}
    \caption{\summac zero-shot balanced accuracy. The hypothesis aggregation method (\S\ref{sec:multi_sent_hyp}) is in parenthesis.}
    \label{tab:summac}
\end{table*}

The \summac benchmark includes six datasets: CGS~\citep{falke-etal-2019-ranking},
XSF~\citep{maynez-etal-2020-faithfulness},
Polytope~\citep{huang-etal-2020-achieved},
FactCC~\citep{kryscinski-etal-2020-evaluating},
SummEval~\citep{fabbri-etal-2021-summeval},
Frank~\citep{pagnoni-etal-2021-understanding}.

Table~\ref{tab:summac} reports the results on this benchmark. See \S\ref{sec:res_ret_cls} for discussion.


\section{Additional Details on the Wiki Clusters Dataset}\label{sec:wikiclusters_details}


As described in Section~\ref{sec:wiki_clusters}, we created a Wikipedia-based dataset with clusters of similar articles written by different communities in multiple languages. Below, we provide additional details on the process.

We first collect the 5000 most popular accessed pages in the English Wikipedia, according to the ranking of November 2021.\footnote{\url{https://bit.ly/Wiki_popular_pages}}
We take a cleaned version (without links) of the introduction of each page (the text coming before the content table). Then, to create the cluster for each article, we use each article's language links and collect similar introductions from the 10 (non-EN) languages that with most admins as of November 2021.\footnote{By \url{https://en.wikipedia.org/wiki/List_of_Wikipedias\#Edition_details}: DE, FR, IT, PL, RU, SV, ZH, ES, PT, UK.}
Finally, we use Google Translate API to translate all articles to English. 

We manually examine a random subset of the clusters and find very few translation mistakes and that in most clusters there are at least several non-English introductions with sufficient length and content. This is mostly thanks to our choice of popular pages and languages. We also tried to randomly sample English articles but find many of the versions in other languages to be missing or have a single sentence.

As mentioned in Section~\ref{sec:wiki_clusters}, we designed a controlled experiment where we simulate local corruptions to the English version, and use the information from the other versions to predict which sentence was changed. To make the corruptions realistic and not obvious, we rely on the Wikipedia edits collection from the VitaminC test set~\cite{schuster-etal-2021-get}. These edits include both real revisions from Wikipedia history logs, and synthetic edits created by annotators to modify certain facts. To ensure that we only use edits that present a factual modification, we only take pairs of evidence from the same page that are paired with the same claim, but express an opposing relation (one supports it and the other refutes it).

To match the edits from VitaminC with our current version, we use word-level (also splitting hyphens) Jaccard similarity. First, looking from small edits, we only take the VitaminC edit instances with similarity greater than $0.25$ between the ``before'' ($x_{b}$) and ``after'' ($x_{a}$) sentences. Then, for each of the edits, we look for the sentence $x$ from the current article that has the highest Jaccard similarity with either the $x_{b}$ or $x_{a}$ sentence. If no sentence has greater than $0.2$ similarity, we skip this edit. Finally, to decide which of the two sentences is coherent with the current version, we pick the one with the higher Jaccard similarity with $x$. Accordingly, we assume that the other sentence represent a factual modification to the current article, and therefore create a local discrepancy by replacing it with $x$.

Following this process, we obtain a total of 824 local corruptions to 144 different articles. See Table~\ref{tab:wiki_cur_example} for an example.


\begin{table*}[ht]
\centering
\begin{small}
% \begin{minipage}{\linewidth}
        \resizebox{\linewidth}{!}{
% \begin{tabular}{lp{0.15\linewidth}p{0.4\linewidth}p{0.08\linewidth}p{0.12\linewidth}r}
\begin{tabular}{p{0.1\linewidth}|p{0.9\linewidth}}
\toprule
Original & Mars is the site of Olympus Mons, the largest volcano and highest known mountain on any planet in the Solar System, and of Valles Marineris, one of the largest canyons in the Solar System. \\
Corruption & Mars is the site of Olympus Mons, the largest volcano and second-highest known mountain in the Solar System, but far away from Valles Marineris, one of the largest canyons in the Solar System.\\

\midrule
\multicolumn{2}{l}{\emph{Examples of related sentences from other articles with helpful information for identifying the corruption:}} \\
FR & The highest volcano in the Solar System, Olympus Mons (which is a shield volcano), and the largest canyon, Valles Marineris, are found on Mars. \\
IT & Among the most noteworthy geological formations of Mars are: Olympus Mons, or Mount Olympus, the largest volcano in the solar system (27 km high); the Valles Marineris, a long canyon considerably larger than the terrestrial ones; and a huge crater on the northern hemisphere, about 40\% wide of the entire Martian surface. \\
SV & During large parts of Mars' history, long-lasting volcanic eruptions occurred which, among other things, created Olympus Mons, the highest mountain in the solar system.\\

\bottomrule
\end{tabular}
% \end{minipage}
}%
\caption{Example of a \emph{simulated} corruption in the English Wikipedia about Mars from our corrupted articles dataset (\S\ref{sec:wiki_clusters}). We are given the introduction of the English article, consisting of 35 sentences, where one sentence, the ``original'', was replaced with the ``corruption'' one. The goal is to successfully identify which sentence was corrupted by leveraging information from the other 10 related articles (each with 18 sentences on average). We only present the most relevant sentences here, but the model has to read through the whole cluster.}\label{tab:wiki_cur_example}
\end{small}
\end{table*}

==> Cluster NLI paper - revised/sections/app_retrieval.tex <==
\section{Example of NLI vs.\ similarity-based retrieval}
Table~\ref{tab:contract_ret_examples} shows a retrieval example from the ContractNLI dataset, using either SentenceT5 (similarity-based) or \ourmodel (NLI-based) to retrieve spans that might support or refute the candidate hypothesis.

\begin{table*}[t]
\centering
\begin{small}
% \begin{minipage}{\linewidth}
        \resizebox{\linewidth}{!}{
% \begin{tabular}{lp{0.15\linewidth}p{0.4\linewidth}p{0.08\linewidth}p{0.12\linewidth}r}
\begin{tabular}{p{0.09\linewidth}|p{0.9\linewidth}}
\toprule
Hypothesis: & Confidential Information shall only include technical information. $\qquad$ $\qquad$ $\qquad$ \emph{(gold label = contradiction)} \\
\midrule
ST5 top-1 & 5.1.2. use Confidential Information only for the Project;\\
\cmidrule{2-2}
top-2 & 5.3.2. The disclosure of Confidential Information to Recipient or its Representatives shall not give Recipient or its Representatives any licence or other rights in relation to that Confidential Information [...]\\
\midrule
\ourmodel argmax $p_c$ & 3.5. "Confidential information" means any information of whatever form relating to the Project or Discloser or any of its Affiliates or Clients, supplied or made available by Discloser or on its behalf to recipient [...] \\
\cmidrule{2-2}
argmax $p_e$ & You the subject-matter expert \\
\bottomrule
\end{tabular}
% \end{minipage}
}%
\caption{ContractNLI evidence retrieval example. The top two retrievals of the SentenceT5 (ST5) model relate to the hypothesis (discussing confidential information), but are do not refute or support it. Alternatively, retrieving by NLI scores is highly informative as the  sentence with max $p_c$ clearly contradicts the hypothesis.}\label{tab:contract_ret_examples}
\end{small}
\end{table*}

==> Cluster NLI paper - revised/sections/app_summac.tex <==
\section{Multi-sentence hypotheses} \label{sec:summac}

Recently, \citet{SummaC} presented the \summac benchmark for predicting the factual consistency of summaries with their source. The benchmark includes the following six datasets: CGS~\citep{falke-etal-2019-ranking},
XSF~\citep{maynez-etal-2020-faithfulness},
Polytope~\citep{huang-etal-2020-achieved},
FactCC~\citep{kryscinski-etal-2020-evaluating},
SummEval~\citep{fabbri-etal-2021-summeval},
FRANK~\citep{pagnoni-etal-2021-understanding}.
We follow the zero-shot setting here as our main focus on this paper is zero-shot applications of NLI models. For fair comparison with the zero-shot setting of \citet{SummaC}, however, we also tune the threshold on the validation set for each dataset, and report the results on the test set. In early exploration we found naive threshold settings to be competitive as well.

Their proposed zero-shot solution is similar to our approach, relying on multi-task sentence-pair NLI models and aggregating the predictions. Their method, however, aims to achieve a single score for the whole summary. Instead, we focus on short hypotheses and on identifying and flagging specific spans that stand out in a collection of related documents. For completeness, we evaluate our \ourmodel model on this benchmark and also experiment the reranking approach for this application.

Specifically, the \summac zero-shot method ($\summac_{\mathrm{ZS}}$) computes the NLI score of each sentence from the summary with each sentence in the document. Then, the final ``factual consistency'' score for the summary is the average over the maximum entailment score ($p_e$) for each sentence of the hypothesis.

To account for the hypothesis aggregation step, we had to slightly adjust our reranking approach. Specifically, we experiment with the following settings:
\begin{itemize}[leftmargin=*]
    \item \textbf{\ourmodel:} We simply replace the backbone NLI model of $\summac_{\mathrm{ZS}}$ with \ourmodel and follow the same aggregation process (without reranking). Hence, the main difference is that we use T5-large~\citep{t5_paper} instead of BERT-large~\citep{devlin-etal-2019-bert}, and possible other small differences regarding the training configuration.
    \item \textbf{+ soft rerank:} For each of the hypothesis sentences, the entailment score is recomputed by running \ourmodel again with both the most supporting and the most contradicting sentences from the document, according to the first-pass NLI scores. Since there is already a $\max$ operation over the scores, this can be viewed as smoothing the score by adding the most contradicting sentence to the context.
    \item \textbf{+ hard rerank:} We perform the following two modifications over the soft method: (1) we use the difference between entailment and contradiction scores from the rerank run ($p_e - p_c$); and (2)
    we set a $\min$ instead of $\mathrm{mean}$ operation, effectively requiring \emph{all sentences} of the hypothesis to be supported.
\end{itemize}


The results are summarized in Table~\ref{tab:summac}. Replacing the backbone model with ours improves the overall performance by absolute $1.2$ points. This overall improvement comes despite a drop of almost 10 points on the Polytope dataset. We note that the ``factual consistency'' definitions used for \summac label summaries with ``addition'' (of unnecessary content) or ``omission'' errors as negative. These errors related more to the quality of the summary rather to its correctness. Therefore, we do not expect zero-shot NLI models to them. 

The effectiveness of reranking varies by dataset. The best overall performance is achieved with hard reranking, improving over the previous aggregation in 4 out of the 6 datasets, and obtaining an overall gain of $0.2$ points.


\begin{table*}[t]
\small
    \centering
    \begin{tabular}{l|dddddd|d}
    \toprule
    Method & \multicolumn{1}{c}{CGS} & \multicolumn{1}{c}{XSF} & \multicolumn{1}{c}{Polytope}& \multicolumn{1}{c}{FactCC} & \multicolumn{1}{c}{SummEval}& \multicolumn{1}{c}{FRANK} & \multicolumn{1}{c}{Overall}\\
    % \cmidrule{2-4}
    \midrule
    $\summac_{\mathrm{ZS}}$ & 70.4 & 58.4 & \textbf{62}.\textbf{0} & 83.8 & 78.7 & 79.0 & 72.1 \\
    \midrule
    \ourmodel & 79.3 & 59.3 & 52.4 & \textbf{89}.\textbf{5} & 77.2 & \textbf{82}.\textbf{1} & 73.3 \\
    + soft rerank & 79.6 & 62.7 & 52.8 & 86.1 & 78.5 & 80.4 & 73.3 \\
    + hard rerank & \textbf{80}.\textbf{5} & \textbf{64}.\textbf{2} & 55.1 & 83.3 & \textbf{79}.\textbf{7} & 78.4 & \textbf{73}.\textbf{5} \\ 
     \bottomrule
    \end{tabular}
    \caption{Balanced accuracy of zero-shot methods on the \summac benchmark.}
    \label{tab:summac}
\end{table*}

==> Cluster NLI paper - revised/sections/app_technical.tex <==
\section{Implementation details for \ourmodel} \label{sec:technical_det}

We use the T5X framework~\citep{roberts2022scaling} to finetune the T5.1.1-Large model for 500K steps and pick the best performning checkpoint on the evaluation splits of the source datasets. We use a batch size of 128 with a balanced sampling across the training datasets to account for their different sizes.

==> Cluster NLI paper - revised/sections/app_wiki.tex <==
\section{Examples of discrepancies and consensus in Wikipedia}\label{sec:wiki_examples}

We present the retrievals of our method for identifying discrepancies and consensus in document clusters (\S\ref{sec:wiki_clusters}) when applied on the ``Dracula'' (Tables~\ref{tab:dracula_dis}-\ref{tab:dracula_con}), ``Big Ben'' (Tables~\ref{tab:bigben_dis}-\ref{tab:bigben_con}), and ``Cameron Boyce'' (Tables~\ref{tab:cameron_dis}-\ref{tab:cameron_con}) pages.
We observe that in general shorter sentences with consensus tend to be short and concise. This is intuitive as longer sentence are more likely to include claims that are missing from other documents.


\begin{table*}[ht]
\centering
\begin{small}
% \begin{minipage}{\linewidth}
        \resizebox{\linewidth}{!}{
% \begin{tabular}{lp{0.15\linewidth}p{0.4\linewidth}p{0.08\linewidth}p{0.12\linewidth}r}
\begin{tabular}{p{0.05\linewidth}|p{0.95\linewidth}}
\multicolumn{2}{l}{\emph{Dracula: searching for \textbf{discrepancies}.}} \\
\toprule
FR & Dracula is an epistolary novel by British writer Bram Stoker published in 1897. \\
\midrule
\multicolumn{2}{l}{\emph{Top sentence from each document by disagreement with the candidate:}} \\
EN & A small group, led by Abraham Van Helsing, hunt Dracula and, in the end, kill him.\\
DE & Dracula is a novel by Irish writer Bram Stoker published in 1897.\\
IT & Dracula is an epistolary novel written by Irish Bram Stoker in 1897, inspired by the figure of Vlad III, prince of Wallachia, and is one of the last examples of Gothic novels.\\
PL & Dracula - a 19th-century Gothic novel by the Irish writer Bram Stoker, depicting the fight of a group of volunteers with the vampire Dracula.\\
RU & Dracula is a novel by the Irish writer Bram Stoker, first published in 1897.\\
PT & Dracula (Dracula) is an 1897 gothic horror novel written by Irish author Bram Stoker, starring the vampire Count Dracula.\\
ES & Dracula is a novel published in 1897 by the Irishman Bram Stoker, as a result of which his antagonist character, Count Dracula, became the quintessential Western vampire archetype, becoming considered the most famous vampire.\\
ZH & "Dracula" is a gothic horror novel based on vampires published in 1897 by Irish writer Bram Stoker.\\
SV & Dracula is a horror novel from 1897 by the Irish author Bram Stoker, in which the main antagonist is the vampire Count Dracula.\\
UK & Dracula is a novel by Irish writer Bram Stoker, first published in 1897.\\
\bottomrule
\end{tabular}
% \end{minipage}
}%
\caption{The sentence with highest discrepancy score (shown at the top) among all 53 sentences from ``Dracula'' articles. Beneath, we show the sentence from each Wikipedia version that had the highest disagreement score with the candidate. This example is also illustrated in Figure~\ref{fig:intro}.}\label{tab:dracula_dis}
\end{small}
\end{table*}


\begin{table*}[ht]
\centering
\begin{small}
% \begin{minipage}{\linewidth}
        \resizebox{\linewidth}{!}{
% \begin{tabular}{lp{0.15\linewidth}p{0.4\linewidth}p{0.08\linewidth}p{0.12\linewidth}r}
\begin{tabular}{p{0.05\linewidth}|p{0.95\linewidth}}
\multicolumn{2}{l}{\emph{Dracula: searching for \textbf{consensus}.}} \\
\toprule
EN & Dracula is a novel by Bram Stoker, published in 1897. \\
\midrule
\multicolumn{2}{l}{\emph{Top sentence from each document by agreement with the candidate:}} \\
DE & Dracula is a novel by Irish writer Bram Stoker published in 1897. \\
FR & Dracula is an epistolary novel by British writer Bram Stoker published in 1897. \\
IT & Dracula is an epistolary novel written by Irish Bram Stoker in 1897, inspired by the figure of Vlad III, prince of Wallachia, and is one of the last examples of Gothic novels.\\
PL & Dracula - a 19th-century Gothic novel by the Irish writer Bram Stoker, depicting the fight of a group of volunteers with the vampire Dracula.\\
RU & Dracula is a novel by the Irish writer Bram Stoker, first published in 1897.\\
PT & Dracula (Dracula) is an 1897 gothic horror novel written by Irish author Bram Stoker, starring the vampire Count Dracula.\\
ES & Dracula is a novel published in 1897 by the Irishman Bram Stoker, as a result of which his antagonist character, Count Dracula, became the quintessential Western vampire archetype, becoming considered the most famous vampire.\\
ZH & "Dracula" is a gothic horror novel based on vampires published in 1897 by Irish writer Bram Stoker.\\
SV & Dracula is a horror novel from 1897 by the Irish author Bram Stoker, in which the main antagonist is the vampire Count Dracula.\\
UK & Dracula is a novel by Irish writer Bram Stoker, first published in 1897.\\
\bottomrule
\end{tabular}
% \end{minipage}
}%
\caption{The sentence with the most consensus (shown at the top) among all 53 sentences from ``Dracula'' articles. Beneath, we show the sentence from each Wikipedia version that had the highest agreement score with the candidate.}\label{tab:dracula_con}
\end{small}
\end{table*}


\begin{table*}[ht]
\centering
\begin{small}
% \begin{minipage}{\linewidth}
        \resizebox{\linewidth}{!}{
% \begin{tabular}{lp{0.15\linewidth}p{0.4\linewidth}p{0.08\linewidth}p{0.12\linewidth}r}
\begin{tabular}{p{0.05\linewidth}|p{0.95\linewidth}}
\multicolumn{2}{l}{\emph{Big Ben: searching for \textbf{discrepancies}.}} \\
\toprule
SV & Big Ben is officially called the Great Bell of Westminster and strikes every hour in the tower clock with the official name Great Clock of Westminster. \\
\midrule
\multicolumn{2}{l}{\emph{Top sentence from each document by disagreement with the candidate:}} \\
EN & The official name of the tower in which Big Ben is located was originally the Clock Tower, but it was renamed Elizabeth Tower in 2012, to mark the Diamond Jubilee of Elizabeth II, Queen of the United Kingdom.\\
DE & The tower has been officially called Elizabeth Tower since September 2012.\\
FR & Previously, it was simply called the Clock Tower.\\
IT & This bell tower rings every quarter of an hour.\\
PL & On September 12, 2012, the tower was officially named Elizabeth Tower in honor of Elizabeth II's 60-year reign.\\
RU & The official name of the tower since 2012 is the Elizabeth Tower, one of the most recognizable symbols of Great Britain, often used in souvenirs, advertisements, and movies.\\
PT & The official name of the tower in which Big Ben is located was originally Clock Tower, but it was renamed Elizabeth Tower in 2012 to mark Queen Elizabeth II's Diamond Jubilee.\\
ES & Its official name was Clock Tower, until on June 26, 2012, in honor of Queen Elizabeth II's Diamond Jubilee, it was decided that the tower would be renamed Elizabeth Tower.\\
ZH & Big Ben (English: Big Ben, or translated as Big Ben) is a big newspaper clock located at the north end of the Palace of Westminster in London.\\
UK & The official name of the tower since 2012 - Elizabeth Tower (English Elizabeth Tower).\\
\bottomrule
\end{tabular}
% \end{minipage}
}%
\caption{The sentence with second highest discrepancy score (shown at the top) among all 72 sentences from ``Big Ben'' articles. Beneath, we show the sentence from each Wikipedia version that had the highest disagreement score with the candidate.}\label{tab:bigben_dis}
\end{small}
\end{table*}

\begin{table*}[ht]
\centering
\begin{small}
% \begin{minipage}{\linewidth}
        \resizebox{\linewidth}{!}{
% \begin{tabular}{lp{0.15\linewidth}p{0.4\linewidth}p{0.08\linewidth}p{0.12\linewidth}r}
\begin{tabular}{p{0.05\linewidth}|p{0.95\linewidth}}
\multicolumn{2}{l}{\emph{Big Ben: searching for \textbf{consensus}.}} \\
\toprule
UK & The official name of the tower since 2012 - Elizabeth Tower (English Elizabeth Tower). \\
\midrule
\multicolumn{2}{l}{\emph{Top sentence from each document by agreement with the candidate:}} \\
EN & The official name of the tower in which Big Ben is located was originally the Clock Tower, but it was renamed Elizabeth Tower in 2012, to mark the Diamond Jubilee of Elizabeth II, Queen of the United Kingdom.\\
DE & The tower has been officially called Elizabeth Tower since September 2012.\\
FR & The tower was renamed on the occasion of the Diamond Jubilee of Elizabeth II in 2012.\\
IT & Known as the Clock Tower, the name was officially changed to Elizabeth Tower on the occasion of Elizabeth II's Diamond Jubilee in June 2012.\\
PL & On September 12, 2012, the tower was officially named Elizabeth Tower in honor of Elizabeth II's 60-year reign.\\
RU & The official name of the tower since 2012 is the Elizabeth Tower, one of the most recognizable symbols of Great Britain, often used in souvenirs, advertisements, and movies.\\
PT & The official name of the tower in which Big Ben is located was originally Clock Tower, but it was renamed Elizabeth Tower in 2012 to mark Queen Elizabeth II's Diamond Jubilee.\\
ES & Its official name was Clock Tower, until on June 26, 2012, in honor of Queen Elizabeth II's Diamond Jubilee, it was decided that the tower would be renamed Elizabeth Tower.\\
ZH & Big Ben (English: Big Ben, or translated as Big Ben) is a big newspaper clock located at the north end of the Palace of Westminster in London.\\
SV & The tower, which has been called Elizabeth Tower since 2012 and where the clock hangs, is 96.3 meters high.\\
\bottomrule
\end{tabular}
% \end{minipage}
}%
\caption{The sentence with the most consensus (shown at the top) among all 72 sentences from ``Big Ben'' articles. Beneath, we show the sentence from each Wikipedia version that had the highest agreement score with the candidate.}\label{tab:bigben_con}
\end{small}
\end{table*}


\begin{table*}[ht]
\centering
\begin{small}
% \begin{minipage}{\linewidth}
        \resizebox{\linewidth}{!}{
% \begin{tabular}{lp{0.15\linewidth}p{0.4\linewidth}p{0.08\linewidth}p{0.12\linewidth}r}
\begin{tabular}{p{0.03\linewidth}|p{0.98\linewidth}}
\multicolumn{2}{l}{\emph{Cameron Boyce: searching for \textbf{discrepancies}.}} \\
\toprule
UK & He died of an epileptic seizure on the night of July 7, 2019 at 2:35 p.m. \\
\midrule
\multicolumn{2}{l}{\emph{Top sentence from each document by disagreement with the candidate:}} \\
ZH & On July 6, 2019, Boyce died of epileptic seizures at the age of 20.\\
RU & Cameron Mica Boyce (born May 28, 1999 - July 6, 2019) - American actor and dancer, best known for his leading roles in the comedy series Jesse (2011-2015) and Gamer's Diary (2015-2017) , as well as in the series of films "Descendants" (2015-2019).\\
EN & Cameron Mica Boyce (May 28, 1999 – July 6, 2019) was an American actor.\\
PL & Cameron Mica "Cam" Boyce (born May 28, 1999 in Los Angeles, died July 6, 2019 therein) - American actor, dancer and model.\\
FR & Cameron Boyce is an American actor, dancer, singer and model, born May 28, 1999 in Los Angeles (California) and died July 6, 2019 in the same city.\\
ES & Cameron Mica Boyce (Los Angeles, California; May 28, 1999-July 6, 2019) was an American actor known primarily for his roles in the feature films Descendants, Descendants 2, Descendants 3, as well as for his role of Luke Ross on the Disney Channel series Jessie.\\
PT & Cameron Boyce (Los Angeles, May 28, 1999 – Los Angeles, July 6, 2019) was an American actor, singer, dancer and voice actor, known for starring in films such as Mirrors and appearing in Eagle Eye, both of 2008.\\
SV & Cameron Boyce, born May 28, 1999 in Los Angeles, died July 6, 2019 in Los Angeles, was an American actor.\\
DE & Cameron Boyce (born May 28, 1999 in Los Angeles, California - July 6, 2019) was an American actor and child actor.\\
IT & Cameron Mica Boyce (Los Angeles, May 28, 1999 - Los Angeles, July 6, 2019) was an American actor and dancer.\\
\bottomrule
\end{tabular}
% \end{minipage}
}%
\caption{The sentence with highest discrepancy score (shown at the top) among all 38 sentences from ``Cameron Boyce'' articles. Beneath, we show the sentence from each Wikipedia version that had the highest disagreement score with the candidate.}\label{tab:cameron_dis}
\end{small}
\end{table*}


\begin{table*}[ht]
\centering
\begin{small}
% \begin{minipage}{\linewidth}
        \resizebox{\linewidth}{!}{
% \begin{tabular}{lp{0.15\linewidth}p{0.4\linewidth}p{0.08\linewidth}p{0.12\linewidth}r}
\begin{tabular}{p{0.03\linewidth}|p{0.98\linewidth}}
\multicolumn{2}{l}{\emph{Cameron Boyce: searching for \textbf{consensus}.}} \\
\toprule
EN & Cameron Mica Boyce (May 28, 1999 – July 6, 2019) was an American actor. \\
\midrule
\multicolumn{2}{l}{\emph{Top sentence from each document by agreement with the candidate:}} \\
PL & Cameron Mica "Cam" Boyce (born May 28, 1999 in Los Angeles, died July 6, 2019 therein) - American actor, dancer and model.\\
RU & Cameron Mica Boyce (born May 28, 1999 - July 6, 2019) - American actor and dancer, best known for his leading roles in the comedy series Jesse (2011-2015) and Gamer's Diary (2015-2017) , as well as in the series of films "Descendants" (2015-2019).\\
ES & Cameron Mica Boyce (Los Angeles, California; May 28, 1999-July 6, 2019) was an American actor known primarily for his roles in the feature films Descendants, Descendants 2, Descendants 3, as well as for his role of Luke Ross on the Disney Channel series Jessie.\\
IT & Cameron Mica Boyce (Los Angeles, May 28, 1999 - Los Angeles, July 6, 2019) was an American actor and dancer.\\
ZH & Cameron Mica Boyce (English: Cameron Mica Boyce, May 28, 1999-July 6, 2019) was an American actor and dancer.\\
PT & Cameron is best known for playing Luke Ross in Jessie, a series that aired on the Disney Channel, and for his role in the film Descendants, having also played the role of Conor in Gamer's Guide to Pretty Much Everything.\\
SV & Boyce was known for his roles in films such as Mirrors, Eagle Eye, Grown Ups and Grown Ups 2.\\
FR & Cameron Boyce is an American actor, dancer, singer and model, born May 28, 1999 in Los Angeles (California) and died July 6, 2019 in the same city.\\
DE & Cameron Boyce (born May 28, 1999 in Los Angeles, California - July 6, 2019) was an American actor and child actor.\\
UK & Cameron Boyce is an American actor and dancer best known for his roles in the feature films "Mirrors," "Hook," "Classmates," "Heirs," "Heirs 2" and the Disney series Jesse.\\
\bottomrule
\end{tabular}
% \end{minipage}
}%
\caption{The sentence with the most consensus (shown at the top) among all 38 sentences from ``Cameron Boyce'' articles. Beneath, we show the sentence from each Wikipedia version that had the highest agreement score with the candidate.}\label{tab:cameron_con}
\end{small}
\end{table*}

==> Cluster NLI paper - revised/sections/beyond_sent.tex <==
\section{Beyond Sentence-level Inference}\label{sec:beyond_sent}


% In the following, we develop and evaluate methods that build on this model for realistic use cases beyond sentence-pair inputs.  \tal{zzz}

We now assume that our target application requires the evaluation of hypotheses against \emph{long texts}. 
We also assume that we have limited or no training data for this domain, and focus on \emph{zero-shot} transfer.
Formally, we assume that $\prem$ is a document consisting of $n$ sentences $S_{1:n}$ and we don't know which part of the document is most relevant for verifying or rejecting $\hyp$. 
% This is a common practical setting where the user is interested in knowing whether a document agrees or contradicts with a specific statement.
In this case, it is common to not only classify the truthfulness of the given statement, but to also point to the exact evidence in the document that led to this conclusion. 
% In this case, it is likely that the user will require the automated system to not only predict the relation between the statement and the document, but to also point to the exact evidence from the document that led to this conclusion. 
This is a crucial requirement, both benefiting the interpretability and trustworthiness of the model (e.g., avoiding hypothesis-only bias), and saving human time needed for manual prediction verification.
% Interpreting the model's predictions is crucial for both efficiently verifying the output (e.g., ensuring no hypothesis-only bias~\citep{gururangan-etal-2018-annotation,poliak-etal-2018-hypothesis, schuster-etal-2019-towards}), and to assist the user in providing justifications to a third-party.


\subsection{Na\"ive premise truncation}
A na\"ive design choice for such applications would be to simply use a similar cross-attention model and provide as much as possible from the input text. As Transformer models are trained with a defined maximum input length limit (typically 512 tokens), this approach has obvious limitations. Yet, in some applications we can assume where the relevant information is likely to be and remove the rest. For example, \citet{yin-etal-2021-docnli} found a model that truncates the input to even outperform a model that supports long inputs on DocNLI. 
% Also, Transformers can potentially generalize to longer inputs at inference~\citep{press2021train}.

Nevertheless, this approach is unlikely to suit very long inputs as the complexity of Transformers grows quadratically with the input length~\citep{tay2021long, attention_all_you_need}. Also, this approach doesn't directly support the important interpretability requirement discussed above, as it is unclear which part of the long document led the model to its prediction.


% Following our observation that models can generalize beyond the length of training examples (\S\ref{sec:docnli_by_len}), one might consider simply increasing the limit during inference. However, there are several downsides to this approach. 

% First, as Figure~\ref{fig:docnli_by_len} shows, the performance starts decreasing even before reaching the length limit. Second, due to the quadratic relation between the cost of the self-attention layer and the sequence length~\citep{tay2021long, attention_all_you_need}, increasing the length of the input has significant impact on memory consumption and latency. Lastly, this approach doesn't directly support the important interpretability requirement discussed above as it is unclear which part of the long document led the model to its prediction.



% \citet{yin-etal-2021-docnli} found a model with an input limit of 512 tokens to perform well on DocNLI, by simply truncating the remainder of the input.
% We follow their setting and evaluate a na\"ive zero-shot application of \ourmodel on this new domain. Table~\ref{tab:res_docnli} shows that \ourmodel performs much better than a random baseline and is competitive with some of the supervised models, indicating promising transfer potential.

% This suggests that \ourmodel is basing its predictions on features that are general enough to transfer to new domains and settings.

% , suggesting that the relevant information for prediction mostly appears at the beginning of the premise. 

\subsection{Retrieve-and-classify over long premises}
% \subsection{Full-document premise for a hypothesis sentence: Retrieve-and-classify}
\label{sec:ret-and-cls}

Instead, we opt to break the long premise into individual sentences and make pointwise predictions against the hypothesis before aggregating them to the final classification. This approach can readily extend to any document length without modifications to the core NLI model. Also, in zero-shot transfer, this allows better alignment with the sentence-pair training distribution. While it requires $n$ inference runs of the NLI model instead of a single pass, the cost increases linearly with $n$, unlike the quadratic effect of increasing the input length. Also, these inference passes can be computed in parallel with batches.
% , reducing the overall latency and flexibly controlling for memory usage.

This pointwise approach, however, has some limitations. First, it requires a robust sentence-pair model that can separate neutral sentences from relevant ones. Second, it doesn't immediately support multi-hop inference over multiple sentences~\citep{jiang-etal-2020-hover}.  This can be partially alleviated with preprocessing techniques \cite[e.g.,][]{choi-etal-2021-decontextualization}. In practice, we don't observe this limitation in our explored applications as most sentences in these domains are sufficiently self-contained (see Figure~\ref{fig:intro}).

Next, we discuss methods for performing the two key steps of the retrieve-and-classify approach.

\subsubsection{Retrieval}\label{sec:retrieval}
Given the long multi-sentenced premise, we would like to identify which sentences are most helpful for accepting or rejecting the hypothesis. We focus on methods supporting data-sparse target domains. 

\newpar{Similarity-based retrieval.}
Most unsupervised retrievers use a similarity function (e.g., inner product) over sparse or dense representations to compare $\hyp$ and each of the premise sentences.

\newpar{NLI-based retrieval.}
We introduce an alternative retrieval approach where we use the non-neutral scores of an NLI model to determine the usefulness of a sentence for classifying the hypothesis. This is motivated by the fact that two neutral sentences can be very similar by many measures, but uninformative for our purpose, such as, e.g., $\prem=$``$\textit{We discuss later whether } \hyp$''. 

% Unlike similarity-based retrieval, 
Here, each sentence ends up having two ranking scores with respect to the hypothesis: for entailment and for contradiction. As we see next, this granularity is useful for downstream steps such as reranking or reasoning over clusters.

% To construct a final prediction, we define the following two methods:

\subsubsection{Classification}
Following the evidence retrieval, we define two methods for constructing the final prediction:

% We are now equipped to perform both evidence retrieval and classification with the same sentence-pair NLI model. First, we compute the pairwise $p_{y,i}$ scores for $\hyp$ against each span $S_i$. 
% We define two methods for constructing the final prediction:


\newpar{Retrieve-and-Predict.}
Assuming NLI-based retrieval, we can simply reuse the same scores.
We pick the span with the strongest score for each label, $\bar{p_y} = \max_{i \in [1,n]}{(p_{y,i})}$, and then predict by the highest NLI score: 
% \vspace{-.5em}
\begin{equation*}
\begin{small}
\text{prediction} =
\left\{
	\begin{array}{ll}
		\argmax_y \bar{p_y}  & \mbox{if } \max_{y\in \{e, c\}} \bar{p_y} > T,  \\
		\text{'neutral'} & \mbox{otherwise.}
	\end{array}
\right.
\end{small}
% \vspace{-.5em}
\end{equation*}
We simply set $T=0.5$ for the zero-shot setting, but it can be potentially tuned. Effectively, the prediction is determined by the span with the strongest sentiment towards the hypothesis.



\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/nli_rerank_2c.pdf}
      \vspace{-16pt}
    \caption[]{NLI-based retrieve-and-rerank concatenates the K spans with the strongest 'entail' score, and the K with the strongest 'contradict' score for reranking, as long as some span's non-neutral score exceeds $T$.}
      \vspace{-8pt}
    \label{fig:rerank}
\end{figure}

\newpar{Retrieve-and-Rerank.}
Instead of directly using the retrieval scores, we rerun the same NLI model on the original hypothesis, and a concatenation of the top-K spans retrieved for both non-neutral labels. For symmetry, we average over two instances: the first concatenating the top-entailing spans in score order, then the top-contradicting spans; and the second instance switching the entailing and contradicting spans. Figure~\ref{fig:rerank} illustrates this process with $K=2$.

This reranking allows the NLI model to directly contrast the spans that are most entailing with the spans that are most contradicting toward the hypothesis.
The resultant multi-sentence premise is longer than the training distribution. Yet, we find \ourmodel to generalize well to slightly longer but focused premises.

% Motivated by our earlier findings (\S\ref{sec:docnli_by_len}), we expect the model to generalize to this slightly longer but focused premise.
% This focused comparison creates a short two-sentence premise that is still relatively close to the training distribution of sentence-pair models.

% \subsection{Full-document premise for a multi-sentence hypothesis}
\subsection{Multi-sentence hypotheses}
\label{sec:multi_sent_hyp}


NLI models could also be useful in scoring texts that are longer than a single focused statement. Recently, \citet{SummaC} used NLI scores to predict the faithfulness of generated summaries with respect to their source. Here, we can break both the premise (e.g., the source) and the hypothesis (the summary) into spans, retrieve-and-classify (with or without reranking) for each hypothesis span, and aggregate.
We consider two methods for aggregating the scores of the hypothesis spans:

\newpar{Soft aggregation.}
Following \citet{SummaC}, we take the average entailment scores across spans. When using our reranking method, we take the shifted difference between the scores: $p_e - p_c + T$.
% follow summac, but with rerank

\newpar{Hard aggregation.}
We take the minimum entailment score across spans, effectively requiring all of the hypothesis spans to be strongly supported.
% replace mean with min.



\subsection{Reasoning over multi-document clusters}\label{sec:clusters_method}


\begin{algorithm}[t]
\small
\caption{Find factual discrepancies in a cluster.}\label{alg:cluster}
\begin{algorithmic}
\Require Cluster of documents $\mathcal{D}$ with spans $\mathcal{S}$, and NLI model.
\Ensure Sorted spans by discrepancy likelihood.
\State $\omega_{i,j} \gets 0 \quad \forall \text{ span } j \text{ in document } i$
\For{$D_i \in \mathcal{D}$}
\For{$S_j \in D_i$}
\State $\hyp \gets S_{i,j}$; $\quad \Omega \gets \{ \}$ 
\For{$D_k \in \mathcal{D} \setminus D_i$}
\State $\Gamma \gets \{ \}$ 
\For{$S_{k,l} \in D_k$}
\State $p_c \gets \text{\ourmodel}(\hyp, S_{k,l})[c]$
\State $\Gamma \gets \Gamma \cup \{p_c\}$
\EndFor
\State $ \Omega \gets \Omega \cup \max(\Gamma)$ 
\EndFor
\State $\omega_{i,j} \gets \mathrm{mean}(\Omega)$ 
% \State $\omega_{i,j} \gets \sum(\Omega)/ |\Omega|$ 
\EndFor
\EndFor
\Return $\mathcal{S}$ sorted by respective $\omega$
\end{algorithmic}
\end{algorithm}


\begin{table*}[t]
\small
    \centering
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{c|c|cccc}
        \toprule
        Eval dataset & \multicolumn{0}{c}{Hypothesis length} & \multicolumn{0}{|c}{Premise length} & Docs per premise & \multicolumn{0}{c}{Sents per doc} & \multicolumn{0}{c}{Sentence length}\\
        \midrule
        DocNLI (-ANLI) \citep{yin-etal-2021-docnli} & 98.91 (52-144) & 530.24 (70-1312) &  1 & 17.53 (3 - 43)  & 30.47 (12-51)
 \\ % 17.53$\pm$23.47
        ContractNLI  \citep{koreeda-manning-2021-contractnli-dataset} & 19.35 (11-27) & 2408.75 (939-4409) & 1 & 79.63 (36 - 128) & 30.28 (1-74)
\\ % 79.63$\pm$44.93
        \summac  \citep{SummaC} & 62.63 (22-117) & 678.52 (240-1234) & 1 & 22.16 (8-41) & 30.38 (11-50)\\ % 23.28$\pm$33.80
        Wiki Clusters (Section~\ref{sec:wiki_clusters}) & 34.83 (17-58) & 2498.39 (999-4152) & 9.86 (10-10) & 7.79 (2-16) & 32.52 (13-56)\\
    \bottomrule
    \end{tabular}
        }%
                \vspace{-5pt}
    \caption{Evaluation datasets and the average tokenized lengths (with 10/90th percentiles), number of sentences per premise document, and length of each sentence. The premise in our Wiki clusters consists of multiple documents.}
    \label{tab:eval_datasets}
      \vspace{-10pt}
\end{table*}

So far, we dealt with evaluating a single, short or long hypothesis against a long premise. In some applications, however, the user might not know which hypothesis to check, but rather would like to query over their corpus to identify the most extreme ones. 
% For example, in the news domain we commonly have a collection of articles written by different sources and describing the same event. 
For example, consider a collection of news articles on the same topic written by different sources.
Typical questions to ask about this corpus could be: \emph{``is there any claim made by one article that other articles disagree with?''}, or other queries like \emph{``what is the most controversial claim?''} or \emph{``is there consensus on some claims in the corpus?''}

Answering such questions goes beyond the typical NLI setting and requires understanding a complex many-to-many relation between the documents, involving multiple alignment and reasoning challenges. Therefore, any solution with low signal-to-noise ratio is likely to fail.

Using our robust \ourmodel model, we introduce an algorithm for identifying such claims. 
Algorithm~\ref{alg:cluster} ranks all of the cluster's spans by discrepancy likelihood.\footnote{When looking for consensus, $p_c$ is replaced by $p_e$.}
Each span is compared against all other spans from all documents. The score is determined by the most contradicting pairing from each document and averaged across the cluster. While this procedure requires many calls to the NLI model (quadratic in number and size of documents), they are independent and can easily be batched and parallelized. 

% Following our promising findings on the robustness of \ourmodel, we rely on it to construct a cluster-level algorithm for answering these queries. 





==> Cluster NLI paper - revised/sections/clusters.tex <==
\section{Analyzing Document Clusters}\label{sec:clusters}
So far, we dealt with evaluating a single, short or long hypothesis against a long premise. In some applications, however, the user might not know which hypothesis to check, but rather would like to query over their corpus to identify the most extreme ones. 
% For example, in the news domain we commonly have a collection of articles written by different sources and describing the same event. 
For example, consider a collection of news articles on the same topic written by different sources.
Typical questions to ask about this corpus could be: \emph{``is there any claim made by one article that other articles disagree with?''}, or other aggregations like \emph{``what is the most controversial claim?''} or \emph{``is there consensus on some claims in the corpus?''}

Answering such questions goes beyond the typical NLI setting and requires understanding a complex many-to-many relation between the documents, involving multiple alignment and reasoning challenges. Therefore, any solution with low signal-to-noise rate is likely to fail. Following our promising findings on the robustness of \ourmodel, we rely on it to construct a cluster-level algorithm for answering these queries. 

To test this setting, we create a dataset with clusters of popular Wikipedia articles on the same topic written in different languages, translated to English. Each version of Wikipedia is managed by a different community, leading to occasional disagreements or mistakes~\citep{unified_wiki}, or even the risk of version-specific conspiracy theories.\footnote{\url{www.bbc.com/news/technology-59325128}} We would like to create a system that can scan these articles and find discrepancies, potentially flagging instances to be checked by content moderators.

\subsection{Wikipedia clusters evaluation dataset}\label{sec:wiki_clusters}
We create clusters of introductions to popular Wikpedia articles about the same topic but written by different communities in multiple (up to 11) languages. 
To simplify the setting, we translate all introductions to English with Google Translate API. See App.~\ref{sec:wikiclusters_details} for more details.

For each cluster, we are interested in identifying claims that appear in at least one article and disagree with most other articles. To this end, we examine two settings:

\paragraph{Corrupted articles.}
We synthetically corrupt the English version of each article by inserting a local edit to one of the sentences. The task is to use the other articles of that cluster to identify the sentence that was changed. While it is possible that all other articles don't mention any information about the specific corrupted fact, thanks to the popularity of the chosen articles and languages we find that mostly at least one of the articles includes sufficient information to refute the corrupted sentence. 

To create the corruptions, we use the edits from the test set of the VitaminC dataset~\citep{schuster-etal-2021-get} that express opposite relations towards a mutual claim. 
In total, we create 824 instances based on 144 different topics. In each instance, we corrupt a single sentence from one of the English articles, and provide the 10 related articles from other languages to help identify which fact was changed.

We note that \ourmodel observed Wikipedia sentences (from other articles) in the training mixture. However, they were only used as the premise, whereas here they also represent the hypothesis.

\paragraph{Real discrepancies.}
We test our method in-the-wild, looking for discrepancies in current Wikipedia. Here, we search across all pages in a cluster and look for sentences that disagree with most other pages. Due to the dynamic nature of Wikipedia and since we lack annotations, we use qualitative evaluation and focus on precision of top-ranked sentences rather than recall.

% Since Wikipedia is constantly edited and updated, we use qualitative evaluation and focus on precision rather than recall.



\subsection{Identifying factual discrepancies}
Algorithm~\ref{alg:cluster} describes our approach for ranking the spans across all cluster documents according to their likelihood of being a discrepancy.\footnote{When looking for consensus, $p_c$ is replaced by $p_e$.}
Each span is compared against all other spans from all documents. The score is determined by the most contradicting pairing from each document and averaged across the cluster. While this procedure requires many calls to the NLI model (quadratic in number and size of documents), they are independent and can be easily batched and parallelized. 

\paragraph{Results.}
For our simulated article corruptions, we only rank sentences from the English articles. Table~\ref{tab:wiki_corrupt} reports the results. In addition to our main method, we tried reverse rank by entailment score, but find it to perform even worst than random. We find this to be caused by pairings that support unmodified facts in the corrupted sentence. When ranking by contradiction, \ourmodel performs the best and successfully flags 68\% of the corruptions as its top prediction.

\begin{algorithm}[t]
\small
\caption{Find factual discrepancies in a cluster.}\label{alg:cluster}
\begin{algorithmic}
\Require Cluster of documents $\mathcal{C}$ with spans $\mathcal{S}$, and NLI model.
\Ensure Sorted spans by discrepancy likelihood.
\State $\omega_{i,j} \gets 0 \quad \forall \text{ span } j \text{ in document } i$
\For{$D_i \in \mathcal{C}$}
\For{$S_j \in D_i$}
\State $\hyp \gets S_{i,j}$; $\quad \Omega \gets \{ \}$ 
\For{$D_k \in \mathcal{C} \setminus D_i$}
\State $\Gamma \gets \{ \}$ 
\For{$S_{k,l} \in D_k$}
\State $p_c \gets \text{\ourmodel}(\hyp, S_{k,l})[c]$
\State $\Gamma \gets \Gamma \cup \{p_c\}$
\EndFor
\State $ \Omega \gets \Omega \cup \max(\Gamma)$ 
\EndFor
\State $\omega_{i,j} \gets \mathrm{mean}(\Omega)$ 
% \State $\omega_{i,j} \gets \sum(\Omega)/ |\Omega|$ 
\EndFor
\EndFor
\Return $\mathcal{S}$ sorted by respective $\omega$
\end{algorithmic}
\end{algorithm}



% \paragraph{Discrepancies in-the-wild}
When applying our method on real Wikipedia articles, without any simulated edits, we don't know if there are any current discrepancies. We rank all sentences across all articles in a cluster and inspect the top spans. Surprisingly, even though we took the most popular pages and top moderated languages, our method quickly identified existing inconsistencies. See Appendix~\ref{sec:wiki_examples} for examples.

For instance, as depicted in Figure~\ref{fig:intro}, we find the French Wikipedia to disagree with other versions on the nationality of the author Bram Stoker. \ourmodel ranked this sentence highest among the 53  sentences of that cluster.
Investigating the page's history, this claim was introduced by an edit\footnote{\href{https://fr.wikipedia.org/w/index.php?title=Dracula&diff=133445656&oldid=133334932}{fr.wikipedia.org/w/index.php?title=Dracula\&\\diff=133445656\&oldid=133334932}} in Jan.\ 2017 and remained unchanged for over 5 years.

Interestingly, when looking for consensus and ranking sentences by agreement score, \ourmodel returns the related sentence from the English version that avoids stating the author's nationality: \emph{``Dracula is a novel by Bram Stoker, published in 1897.''} Intuitively, shorter statements have a higher chance of obtaining consensus.

% rank of prediction
In another example, we look at the articles about ``Big Ben''. The top discrepancy prediction was a sentence from the Chinese version that was likely mistranslated due to multiple segmentation options. While this does not necessarily reveal a mistake in the original document, it shows the potential of this approach for flagging translation mistakes when related sources are available. 
The second ranked sentence identifies a statement from the Swedish page regarding the monument's official name. Upon manual verification, even though articles discuss several names that were changed over time, none seem to directly support that claim.


\begin{table}[t]
\small
    \centering
    \begin{tabular}{l|ccc}
    \toprule
    Model & \multicolumn{3}{c}{Accuracy@K} \\
    % \cmidrule{2-4}
    & K=1 & 5 & 10 \\
    \midrule
    Random & 17.11 & 46.53 & 73.68 \\
    \midrule
     \multicolumn{4}{l}{\underline{\textit{Reversed ranking by entailment:}}} \\
    % T5$_{\text{MNLI}}$ & 3.03 & 31.92 & 68.08 \\
    %  T5$_{\text{*NLI}}$ & 8.37 & 48.30 & 76.46 \\
     \ourmodel &1.46 & 17.35 & 40.29 \\
    \midrule
     \multicolumn{4}{l}{\underline{\textit{Ranking by contradiction:}}} \\
    T5$_{\text{MNLI}}$ & 35.32 & 67.60 & 83.37 \\
     T5$_{\text{*NLI}}$ & 38.59 & 70.39 & 83.13 \\
     \ourmodel & \textbf{68.20} & \textbf{89.08} & \textbf{95.15} \\
     \bottomrule
    \end{tabular}
    \caption{Wikipedia corruption detection results by different ranking methods/ models. Accuracy of including the corrupted sentence within the top K predictions.}
    \label{tab:wiki_corrupt}
\end{table}

==> Cluster NLI paper - revised/sections/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
We present a comprehensive study on the performance of sentence-pair NLI models in real world applications that often involve both a shift in domain and long texts. Our findings indicate the readiness of these models to provide meaningful signal on the semantic relation between texts that can be easily aggregated towards practical gains.
To demonstrate this, we also defined a new zero-shot entailment-focused task over clusters of related documents. Our multi-task sentence-pair NLI model (\ourmodel) successfully flags spans that stand out due to their claims.

Ultimately, this study should help practitioners interested in applying NLI-style inference in real-world applications to design the best model for their target task. Our results suggest that if the hypothesis is short and the premise fully fits in the input limit of the model, a regular cross-attention classifier is likely to perform well in terms of accuracy as it is able to contextualize sentences in the premise. However, if we want to interpret the prediction by identifying the exact piece from the premise that led to the predicted conclusion, breaking the premise into segments could be useful. Furthermore, if the premise is too long to fit in the model's receptive field, then breaking the premise into segments and aggregating with our proposed techniques (retrieve-and-classify and reranking) is beneficial. Finally, when we don't have a well defined hypothesis, one might still want to automatically reason over a pair or collection of documents and identify any statements that stand out. In this case,
our reasoning over clusters methodology shows how to use strong sentence-pair classifiers to obtain useful signals that are then aggregated to highlight specific claims.

It's important to note that when designing the methods for this work, we preferred simplicity over performance in order to directly study the quality of the \ourmodel's scores. Yet, we achieve high zero-shot performance and even reach state-of-the-art on ContractNLI. We hope that this work will motivate future research on further expanding these methods, for example by decontextualizing the premise, supporting multi-hop reasoning, expanding the context with sliding windows instead of sentence splitting, or hypothesis fragmentation. 

% formed a new task and developed a baseline that extends current sentence-pair models.

% future work should break down sentences into smaller atomic pieces, and model the context in the specific document.

% opens the door to many exciting opportunities around inspecting collections of free text documents

% We hope that our task and baselines will motivate others to..

==> Cluster NLI paper - revised/sections/eval_datasets.tex <==


\section{Evaluation Tasks and Datasets}\label{sec:eval_tasks}
We evaluate our methods on the following 3 benchmarks that contain 9 datasets from different domains. In addition, we create a new of its kind dataset with clusters of related documents (\S\ref{sec:wiki_clusters}).
The statistics are summarized in Table~\ref{tab:eval_datasets}.

\noindent\textbf{DocNLI}~\citep{yin-etal-2021-docnli} includes long hypotheses and premises, mostly from the news domain. We remove ANLI since it was included in our training data.\footnote{The ANLI examples cover only 1.2\% of the DocNLI test set, so the difference is minimal. \ourmodel and \ourmodel$_{\text{tuned}}$ get .350 and .410 $F_1$ scores on the full test set, respectively.}
Despite the length, a model with input limit of 512 tokens can generally perform well.
%, indicating that the important information is mostly at the beginning of the premise.

% For this experimentation, we use the DocNLI dataset~\citep{yin-etal-2021-docnli} and remove ANLI from it since ANLI was included in our training data.\footnote{The ANLI examples cover only 1.2\% of the DocNLI test set, so the difference is minimal. \ourmodel and \ourmodel$_{\text{tuned}}$ get .350 and .410 $F_1$ scores on the full test set, respectively. } 
% A large portion of DocNLI is based on news articles where the hypothesis is a short summary of an article and the premise is the article itself. 

DocNLI uses only two classes, ``entail'' vs.\ ``not entail''.
% , by merging the ``neutral'' and ``contradiction'' definitions. 
We discuss different zero-shot conversion techniques from 3-way models to binary classification in Appendix~\ref{sec:binary_aggr}.
% The ``not entail'' instances are created with both rule-based and LM-based local perturbations over the positive pairs. This results in a slightly different task definition than NLI since even altered (i.e., ``fake'') texts can still factually agree with the hypothesis~\citep{schuster-etal-2020-limitations}. \citet{yin-etal-2021-docnli} account for this by augmenting the training set, but zero-shot NLI models might be affected by this provenance-based rather than factual-based partition of the test set.


\noindent\textbf{ContractNLI}~\citep{koreeda-manning-2021-contractnli-dataset} has NLI examples in the legal domain. Each hypothesis is short and focused, but the premise is a long document (80 sentences on average). A model with input limit of 512 tokens performs poorly here.

%  We use the ContractNLI dataset~\citep{koreeda-manning-2021-contractnli-dataset} as our main testbed for this part. Unlike the DocNLI data where models with limited input length were shown to perform well, simply truncating ContractNLI inputs to 512 tokens leads to random results. As the documents in ContractNLI contain 80 sentences on average, this setting presents two challenges: (1) identifying and retrieving the relevant evidence sentences per hypothesis, and (2) making the final prediction.
% We will also revisit the long premises of DocNLI and show that this approach is beneficial there as well.
% While we focus here on short hypotheses, in App.~\ref{sec:summac} we evaluate on \summac~\cite{SummaC} with multi-sentence hypotheses.

\noindent\textbf{\summac}~\citep{SummaC} is a benchmark for predicting the factual consistency of summaries with their source.
We follow the zero-shot setting here, but for fair comparison with \citet{SummaC}, we also tune the threshold on the validation set for each dataset, and report the results on the test set. In early exploration we found naive threshold settings to be competitive as well.


\subsection{Wikipedia clusters evaluation dataset}\label{sec:wiki_clusters}

In addition, we create a new dataset for exploring \emph{inference over collections of related articles}.
Specifically, we collect clusters of introductions to popular Wikipedia articles on the same topic written in up to 11 different languages, machine translated to English. 
See App.~\ref{sec:wikiclusters_details} for more details.\footnote{The Wikipedia clusters data is available at: \url{https://github.com/google-research-datasets/wiki-translated-clusters-nli}}

Each version of Wikipedia is managed by a different community, leading to occasional disagreements or mistakes~\citep{iv2021fruit, unified_wiki}, or even the risk of version-specific conspiracy theories.\footnote{\url{www.bbc.com/news/technology-59325128}}
Therefore, automatically comparing and contrasting the information from different articles could be very helpful.
% We examine the two following settings:
% To study this, we examine the two following settings:
We examine both synthetic corruptions and real discrepancies.

% We create clusters of introductions to popular Wikpedia articles about the same topic but written by different communities in multiple (up to 11) languages. 
% To simplify the setting, we translate all introductions to English with Google Translate API. 

% For each cluster, we are interested in identifying claims that appear in at least one article and disagree with most other articles. To this end, we examine two settings:



\newpar{Corrupted articles.}
We simulate a corruption to the English version of each article by inserting a local edit to one of the sentences. The task is to use the other articles of that cluster to identify the sentence that was changed. While it is possible that all other articles don't mention any information about the specific corrupted fact, thanks to the popularity of the chosen articles and languages we find that mostly at least one of the articles includes sufficient information to refute the corrupted sentence. 

To create the corruptions, we use edits from the test set of the VitaminC dataset~\citep{schuster-etal-2021-get} that express opposite relations towards a mutual claim. 
In total, we create 824 instances based on 144 different topics. In each instance, we corrupt a single sentence from one of the English articles, and provide the 10 related articles from other languages to help identify which fact was changed.

We note that \ourmodel observed Wikipedia sentences (from other articles) in the training mixture. However, they were only used as the premise, whereas here they also represent the hypothesis.

\newpar{Real discrepancies.}
We look for discrepancies in-the-wild, searching in current Wikipedia. 
Here, we don't know which article, if any, might include a discrepancy. Therefore, in this setting, we focus on qualitative evaluation and explore whether we can rank all spans from all articles to identify real discrepancies, or consensus.

% will rank all spans from all articles in each cluster by their discrepancy likelihood, and manually examine the top predictions. 

% Here, we search across all pages in a cluster and look for sentences that disagree with most other pages. Due to the dynamic nature of Wikipedia and since we lack annotations, we use qualitative evaluation and focus on precision of top-ranked sentences rather than recall.

% Since Wikipedia is constantly edited and updated, we use qualitative evaluation and focus on precision rather than recall.

==> Cluster NLI paper - revised/sections/experiments.tex <==

\begin{table}[t]
\small
    \centering
    \begin{tabular}{l|cc}
    \toprule
    Model & Dev. & Test \\
    \midrule
    Random & .198 & .199 \\
    \midrule
    \multicolumn{3}{l}{\underline{\textit{supervised:}}} \\
    Longformer-base$^*$~\citep{yin-etal-2021-docnli} & .462 & .444  \\
     Roberta-large~\citep{yin-etal-2021-docnli} & .631 & .613  \\
     T5-large & .642 &.618 \\
     \midrule
    \multicolumn{3}{l}{\underline{\textit{zero-shot:}}} \\
     \ourmodel (no setnence split) & .341 & .345 \\     
     \ourmodel$_{\text{tuned}}$  (no setnence split) & .409  & .408 \\  
     \bottomrule
    \end{tabular}
                   \vspace{-5pt}
    \caption{$F_1$(E) scores on the \textsc{DocNLI}(-ANLI) binary classification dataset. The zero-shot shot predictions are based on a threshold $T$ on the entailment score which is either set to $0.5$ or \emph{tuned} over $0.2\%$ of the dev set. $^*$Longformer's scores are over the full DocNLI.}
    \label{tab:res_docnli}
    \vspace{-8pt}
\end{table}

\section{Experiments}\label{sec:experiments}

We evaluate our inference pipelines against supervised models from DocNLI and ContractNLI, and the zero-shot \summac model, adopting the main evaluation metrics from each paper. We also train T5-large supervised models to directly compare with \ourmodel's zero-shot performance.

DocNLI~\citep{yin-etal-2021-docnli} used a RoBERTa-large~\citep{roberta} model with input limit of 512 tokens and a Longformer-base~\citep{longformer} model.
ContractNLI introduced the SpanNLI~\citep{koreeda-manning-2021-contractnli-dataset} model to process long documents that they train to jointly identify key spans and to make the final verdict.
\summac~\cite{SummaC} used a BERT-large~\citep{devlin-etal-2019-bert} model that was also trained on multiple NLI datasets.

% \subsection{Baselines}
% baselines from papers

\subsection{Zero-shot transfer to new domains}


% \citet{yin-etal-2021-docnli} found a model with an input limit of 512 tokens to perform well on DocNLI, by simply truncating the remainder of the input.
% , suggesting that the relevant information for prediction mostly appears at the beginning of the premise. 
% We follow their setting and evaluate a naive zero-shot application of \ourmodel on this new domain. 

\parhead{DocNLI.} 
Table~\ref{tab:res_docnli} summarizes the results on DocNLI.  
\ourmodel performs much better than a random baseline and is competitive with some supervised models, indicating promising transfer potential.



% \paragraph{Performance by input length.}
% \subsection{Performance by input length} \label{sec:docnli_by_len}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.46\textwidth]{figures/docnli_by_length.png}
        \vspace{-4pt}
    \caption[]{Effect of input length of DocNLI examples when naively using zero-shot \ourmodel \textbf{without sentence splitting} (simply providing the whole document as a single premise). The blue line shows $F_1$ score as a function of hypothesis length ($|\hyp|$). The orange line bins examples by the premise length ($|\prem|$), focusing only on short hypotheses (where $|\hyp|\le20$). For short hypotheses, the performance stays high even beyond the training distribution, but sharply drops around the input length limit of the model.}
    \label{fig:docnli_by_len}
     \vspace{-5pt}
\end{figure}

We also examine the effect of the input length on the performance in Figure~\ref{fig:docnli_by_len}.
First, we see that the performance is highly affected by the length of the hypothesis. \citet{yin-etal-2021-docnli} observed a similar trend even with supervised models. We conjecture that this is due to the natural increase in ambiguity with the hypothesis' length, as it is more likely to include multiple claims that could be questioned. 
% This motivates our inference pipelines in the following sections that focus on concise hypotheses and aggregate when needed.

Second, we look at the performance as a function of the premise length. To focus on examples where the hypothesis is well defined, we only consider cases with a short hypothesis of no more than 20 tokens (total of 5,932 cases from DocNLI(-ANLI) test set). As the orange line shows, \ourmodel performs well on these cases even when the premise is much longer than the inputs that the model was trained on, demonstrating promising potential for zero-shot applications. However, the performance significantly drops when reaching the input length limit, requiring us to truncate the premise.


% \subsection{ContractNLI with oracle spans}


\begin{table}[t]
\small
    \centering
    \begin{tabular}{ll|c|ccc}
    \toprule
    & Model & S.P. & $F_1$(C) & $F_1$(E) & AVG \\
    \midrule
    & Majority vote$^{\ddag}$ &  &.239 & .645 & .442  \\
    \midrule
    % \multicolumn{3}{l}{\underline{\textit{supervised:}}} \\
    \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{\textit{supervised}}}} 
        & SpanNLI-base$^{\ddag}$ & & .657 & .816 & .736 \\
        & SpanNLI-large$^{\ddag}$ & &.620 & .806 & .713 \\
        & T5-large & v &\textbf{.815} & .971 & .893\\ 
        & \ourmodel$_{\text{+ContractNLI}}$ & v & .813 & \textbf{.978} & \textbf{.895}\\
     \midrule
    % \multicolumn{3}{l}{\underline{\textit{zero-shot:}}} \\
    \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\textit{0-shot}}}} 
        &\ourmodel$_{\text{-M.T}}$ & v &.616 & .882 & .749 \\
        & \ourmodel$_{\text{-F.V}}$ & v &.616 & .869& .742 \\
        & \ourmodel & v & \textbf{.661} &\textbf{.904} & \textbf{.782} \\ 
     \bottomrule
    \end{tabular}
    \vspace{-5pt}
    \caption{ContractNLI results with Oracle evidence spans (excluding neutral examples). Sentence-pair models (S.P.), even in zero-shot setting, outperform the SpanNLI model that was trained on long inputs. $^{\ddag}$Results from \citet{koreeda-manning-2021-contractnli-dataset}.}
    \label{tab:contnli_oracle}
    \vspace{-4pt}
\end{table}

\parhead{ContractNLI.} 
We test zero-shot transfer to the legal domain of ContractNLI. To disentangle the effect of input length, we first examine an oracle retriever setting where the premise includes only the few relevant sentences. Table~\ref{tab:contnli_oracle} summarizes the results.
%
Surprisingly, we find our zero-shot sentence-pair models outperform the supervised SpanNLI models. \ourmodel, trained on all five NLI datasets performs the best, demonstrating strong NLI capabilities on this new domain. 

% In , we compare our sentence-pair models, with and without training on ContractNLI, against the SpanNLI model~\citep{koreeda-manning-2021-contractnli-dataset}. SpanNLI was trained with a joint objective for both selecting the evidence spans from the document and making the NLI prediction per hypothesis. The oracle setting disentangles the NLI task from the span selection as the models are provided with the human-selected spans.

% Surprisingly, we find our zero-shot sentence-pair NLI models, which were trained on a different domain, outperform the supervised SpanNLI model. \ourmodel , which was trained on all five NLI datasets performs the best, demonstrating strong NLI capabilities. We also train supervised sentence-pair NLI models using the training data from ContractNLI. To collect neutral evidence for training hypotheses with this label, we randomly select a span from the document. As expected, the sentence-pair supervised models outperform the zero-shot models, where the best model is trained over the five NLI datasets in addition to ContractNLI.
% Overall, this demonstrates the superiority of the sentence-pair setting over joint objective models.






\subsection{NLI vs.\ similarity-based retrieval}\label{sec:res:retrieval}
We use the span-level annotations of ContractNLI to evaluate span retrieval over the premise for NLI. We find \ourmodel's NLI scores to provide a very strong retrieval signal, ranking one of the annotated spans at the top 61\% of the time. A random baseline, in comparison, achieves less than 1\%.


% Given the promising NLI performance of sentence-pair models, we now turn to the task of identifying the relevant evidence per hypothesis in order to devise the full pipeline.
% Our retrieval procedure is based on the same sentence-pair NLI models and uses the $p_e$ and $p_c$ scores of each document span against the hypothesis. We argue that if the model can successfully distinguish neutral from informative relations, we can use these scores for both retrieval and classification. Indeed, we find \ourmodel's NLI scores to provide very strong retrieval signal. 
% \ourmodel ranks one of the annotated spans as the top-1 span 61\% of the time. A random baseline, in comparison, achieves less than 1\%.

% Compared to a random baseline of less than 1\%, the top-ranked span by \ourmodel's NLI scores is one of the human-annotated spans 61\% of the time.

To compare with similarity-based retrievers, we adopt the TF-IDF baseline from \citet{koreeda-manning-2021-contractnli-dataset}, and also extract unsupervised sentence embeddings with BERT-large~\citep{devlin-etal-2019-bert} and SentenceT5-large~\citep{ni2021sentencet5}. 

Table~\ref{tab:contnli_res} shows the precision of each retriever at recall $0.8$ (P@R.8). Unsupervised NLI-based retrieval outperforms similarity-based retrievers. As discussed in \S\ref{sec:retrieval}, we conjecture that this is because some sentences in the document could be very similar to the hypothesis, but neutral towards it.
Table~\ref{tab:contract_ret_examples} shows an example of such case.
%
Within the supervised methods, SpanNLI performs better, perhaps due to only including single random spans for neutral cases in the sentence-pair training data, not utilizing the full document.



\subsection{Retrieve-and-classify}\label{sec:res_ret_cls}

% back to DocNLI results
\parhead{DocNLI.}
We test if our sentence-pair method can improve the low performance over long premises in DocNLI. We focus on examples with a short hypothesis (up to 20 tokens) and long premise (more than 512 tokens). Naively applying \ourmodel on these cases without sentence splitting leads to a low $0.21$ $F_1$ score. Using our retrieve-and-predict approach, the score increases up to $0.41$. Reranking doesn't seem to improve in this case, possibly due to the dataset's two-way classification format.

\parhead{ContractNLI.}
Table~\ref{tab:contnli_res} shows the main results on ContractNLI comparing sentence-pair zero-shot models with both kinds of supervised models. Surprisingly, the zero-shot sentence-pair models are competitive with the supervised SpanNLI model, even outperforming them in $F_1$(C). The supervised \ourmodel, trained also with ContractNLI, performs best overall. Even though its retrieval performance is still behind SpanNLI (\S\ref{sec:res:retrieval}), its final verdict on the hypothesis is better.
% the random sampling of neutral spans that doesn't utilize the full document.

% The rerank approach provides an average increase of $0.1$ $F_1$ points over the naive aggregation with zero-shot \ourmodel.
Reranking significantly improves the performance of zero-shot \ourmodel, increasing the average score by up to 27\%. We observe better performance with larger context ($K=5$).  For the supervised \ourmodel model, reranking provides only marginal gains, and increasing the context is not beneficial.

Overall, we see that sentence-pair models obtain very strong classification performance, even in a zero-shot setting (Table~\ref{tab:contnli_oracle}), while also providing descent retrieval capabilities. We hypothesize that the gap in the retrieval performance could be due to randomly sampling neutral spans instead of utilizing the full document. Augmenting the training set with more and better neutral examples could further close this gap.


\begin{table}[t]
\small
    \centering
        \resizebox{\linewidth}{!}{
    \begin{tabular}{l|c|c|ccc}
    \toprule
    Model & S.P. & P@R.8 & $F_1$(C) & $F_1$(E) & AVG \\
    \midrule
    Majority vote$^{\ddag}$ &  &  - & .083 & .428 & .256 \\
    \midrule
    \multicolumn{3}{l}{\underline{\textit{supervised:}}} \\
        SpanNLI-base$^{\ddag}$ & & .663 & .287 & .765 & .526\\
        SpanNLI-large$^{\ddag}$ & & \textbf{.793} & .357 & \textbf{.834} & .595 \\
        T5-large & v & .575 & .512 & .691 & .601\\ 
        % $\quad$ + rerank & v & - & .519 & .699 \\
        \ourmodel$_{\text{+Cont.NLI}}$ & v & .580 & .521 & .754 & .637\\
        \ + Rerank$_{(K=1)}$ & v  & " & \textbf{.537}  & .741 & \textbf{.639}\\
        \ + Rerank$_{(K=5)}$ & v & " & .520 & .719 & .619 \\
     \midrule
    \multicolumn{3}{l}{\underline{\textit{zero-shot:}}} \\
        TF-IDF$^{\ddag}$ & v & .057 & - & - & -\\
        BERT emb. & v & .083& - & - & - \\
        SentenceT5 & v & .311& - & - & - \\
        \ourmodel$_{\text{-M.T}}$ & v & .397 & .261 & .551 & .406 \\
        % $\quad$ + rerank & v & - & .350 & .639 & .494\\
         \ourmodel$_{\text{-F.V}}$ & v & .397 & .247 & .594 & .420 \\
        %  $\quad$ + rerank & v & - & .341 & .656 & .499\\
         \ourmodel & v & \textbf{.412} & .257 & .573 & .415 \\ 
         \ + Rerank$_{(K=1)}$ & v & " & .363 & \textbf{.659} & .511 \\
         \ + Rerank$_{(K=5)}$ & v & " & \textbf{.404} & .652 & \textbf{.528} \\
     \bottomrule
    \end{tabular}
    }%
    \vspace{-5pt}
    \caption{Evidence retrieval and classification results of both supervised and zero-shot models on ContractNLI test set. Within sentence-pair (S.P.) models, NLI-based retrieval is more precise than similarity retrievers. Supervised S.P.\ models  outperform the joint SpanNLI model in the final classification task thanks to better $F_1$(C). $^{\ddag}$Results from \citet{koreeda-manning-2021-contractnli-dataset}.}
    \label{tab:contnli_res}
    \vspace{-8pt}
\end{table}

\parhead{\summac.}
For evaluating on \summac, we first adopt the zero-shot method of \citet{SummaC} ($\summac_{\mathrm{ZS}}$) and only replace the backbone NLI model with \ourmodel. This improves the performance by absolute $1.2$ points (see Table~\ref{tab:summac}). This overall improvement comes despite a drop of almost 10 points on the Polytope dataset. This could be due to \summac's labeling function that treats summaries with any added or omitted content, compared to the reference, as ``factual inconsistent''. These errors relate more to the summary quality rather than its correctness and therefore, we do not expect zero-shot NLI models to catch them.

Reranking (K=1) is effective for most datasets. The best overall performance is achieved by reranking and hard aggregating the hypothesis sentences, improving over soft aggregation in 4 out of the 6 datasets, and allowing an overall $0.2$ points gain.



\subsection{Factual discrepancies in clusters}\label{sec:res_wiki}
Table~\ref{tab:wiki_corrupt} reports the results on our \textbf{Corrupted Wiki Clusters} dataset (\S\ref{sec:wiki_clusters}). 
In addition to our main method, we tried to reverse rank the spans by entailment score, but find it to perform even worst than random. We find this to be caused by pairings that support unmodified facts in the corrupted sentence. When ranking by contradiction, \ourmodel performs the best and successfully flags 68\% of the corruptions as its top prediction.



% \paragraph{Discrepancies in-the-wild}
Exploring popular \textbf{Real} Wikipedia articles, without any simulated edits our known discrepancies, our method quickly identified existing inconsistencies. We attach examples in Appendix~\ref{sec:wiki_examples} and discuss them briefly here.
%
As depicted in Figure~\ref{fig:intro}, we find the French Wikipedia to disagree with other versions on the nationality of Bram Stoker. \ourmodel ranked this sentence highest among the 53  sentences of that cluster.
Investigating the page's history, this claim was introduced by an edit\footnote{\href{https://fr.wikipedia.org/w/index.php?title=Dracula&diff=133445656&oldid=133334932}{fr.wikipedia.org/w/index.php?title=Dracula}} in Jan.\ 2017 and remained unchanged for over 5 years.

Interestingly, when looking for consensus and ranking sentences by agreement, \ourmodel returns the English version that avoids stating any nationality: \emph{``Dracula is a novel by Bram Stoker, published in 1897.''} Intuitively, shorter statements have higher chance of obtaining consensus.

% rank of prediction
In another example, we look at the articles about ``Big Ben''. The top discrepancy prediction was a sentence from the Chinese version that was likely mistranslated due to multiple segmentation options. While this does not necessarily reveal a mistake in the original document, it shows the potential of this approach for flagging translation mistakes when related sources are available. 
The second ranked sentence identifies a statement from the Swedish page regarding the monument's official name. Upon manual verification, even though articles discuss several names that were changed over time, none seem to directly support that claim.


\begin{table}[t]
\small
    \centering
    \begin{tabular}{l|ccc}
    \toprule
    Model & \multicolumn{3}{c}{Accuracy@K} \\
    % \cmidrule{2-4}
    & K=1 & 5 & 10 \\
    \midrule
    Random & 17.11 & 46.53 & 73.68 \\
    \midrule
     \multicolumn{4}{l}{\underline{\textit{Reversed ranking by entailment:}}} \\
    % T5$_{\text{MNLI}}$ & 3.03 & 31.92 & 68.08 \\
    %  T5$_{\text{*NLI}}$ & 8.37 & 48.30 & 76.46 \\
     \ourmodel &1.46 & 17.35 & 40.29 \\
    \midrule
     \multicolumn{4}{l}{\underline{\textit{Ranking by contradiction:}}} \\
    \ourmodel$_{\text{-M.T}}$ & 35.32 & 67.60 & 83.37 \\
     \ourmodel$_{\text{-F.V}}$ & 38.59 & 70.39 & 83.13 \\
     \ourmodel & \textbf{68.20} & \textbf{89.08} & \textbf{95.15} \\
     \bottomrule
    \end{tabular}
    \caption{Wikipedia corruption detection results by different ranking methods/ models. Accuracy of including the corrupted sentence within the top K predictions.}
    \label{tab:wiki_corrupt}
\end{table}

==> Cluster NLI paper - revised/sections/full_docs.tex <==
\section{Operating Over Full Documents}\label{sec:fulldoc}

In this section, we turn our focus to applications where a specific hypothesis is evaluated against long texts. Formally, we assume that $\prem$ is a document consisting of $n$ sentences $S_{1:n}$ and we don't know which part of the document is most relevant for verifying or rejecting $\hyp$. 
% This is a common practical setting where the user is interested in knowing whether a document agrees or contradicts with a specific statement.
It is common in this case to not only ask for the truthfulness of the given statement, but to also point to the exact evidence in the document that led to this conclusion. 
% In this case, it is likely that the user will require the automated system to not only predict the relation between the statement and the document, but to also point to the exact evidence from the document that led to this conclusion. 
This is a crucial requirement as it both assists in interpreting and trusting the model (e.g., avoiding hypothesis-only bias), and can practically save time when having to manually verify the prediction.
% Interpreting the model's predictions is crucial for both efficiently verifying the output (e.g., ensuring no hypothesis-only bias~\citep{gururangan-etal-2018-annotation,poliak-etal-2018-hypothesis, schuster-etal-2019-towards}), and to assist the user in providing justifications to a third-party.

% 1. performance does go down even before we meet the limit
% 2. this hard constraint makes the model less adaptable inputs of any length
% 3. interpretability limitation
Following our observation that models can generalize beyond the length of training examples (\S\ref{sec:docnli_by_len}), one might consider simply increasing the limit during inference. However, there are several downsides to this approach. 
First, as Figure~\ref{fig:docnli_by_len} shows, the performance starts decreasing even before reaching the length limit. Second, due to the quadratic relation between the cost of the self-attention layer and the sequence length~\citep{tay2021long, attention_all_you_need}, increasing the length of the input has significant impact on memory consumption and latency. Lastly, this approach doesn't directly support the important interpretability requirement discussed above as it is unclear which part of the long document led the model to its prediction.

% breaking benefits:
% 1. flexible to any input form
% 2. aligns well with the training distribution on NLI
% 3. parallel computation
Instead, we opt to break the long document into individual sentences and make point-wise predictions against the hypothesis before aggregating them to the final prediction. This approach can readily extend to any document length without any modification to the core NLI model. Also, this way the model evaluates examples that are more aligned with the sentence-pair training distribution. While it requires $n$ inference runs of the NLI model instead of a single pass, the cost increase is linear in $n$, unlike the option of increasing the input length limit where the increase is quadratic. Also, these inference passes can be computed in parallel with batches to improve efficiency.
% , reducing the overall latency and flexibly controlling for memory usage.

This point-wise approach, however, has some limitations. First, it requires a robust sentence-pair model that can reliably separate neutral sentences from relevant ones. Second, it doesn't immediately support multi-hop inference over multiple sentences~\citep{jiang-etal-2020-hover}.  This can be partially addressed with preprocessing techniques \cite[e.g.,][]{choi-etal-2021-decontextualization}. In practice, we don't observe this limitation in our explored applications as most sentences are self-contained in these domains.
% breaking down limits
% 1. requires robust models (cleaning "neutral")
% 2. doesn't immediately support multi-hop reasoning

\paragraph{Experimental setting.}
 We use the ContractNLI dataset~\citep{koreeda-manning-2021-contractnli-dataset} as our main testbed for this part. Unlike the DocNLI data where models with limited input length were shown to perform well, simply truncating ContractNLI inputs to 512 tokens leads to random results. As the documents in ContractNLI contain 80 sentences on average, this setting presents two challenges: (1) identifying and retrieving the relevant evidence sentences per hypothesis, and (2) making the final prediction.
We will also revisit the long premises of DocNLI and show that this approach is beneficial there as well.
While we focus here on short hypotheses, in App.~\ref{sec:summac} we evaluate on \summac~\cite{SummaC} with multi-sentence hypotheses.


\subsection{ContractNLI with oracle spans}


\begin{table}[t]
\small
    \centering
    \begin{tabular}{ll|c|ccc}
    \toprule
    & Model & S.P. & $F_1$(C) & $F_1$(E) & AVG \\
    \midrule
    & Majority vote$^{\ddag}$ &  &.239 & .645 & .442  \\
    \midrule
    % \multicolumn{3}{l}{\underline{\textit{supervised:}}} \\
    \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{\textit{supervised}}}} 
        & SpanNLI-base$^{\ddag}$ & & .657 & .816 & .736 \\
        & SpanNLI-large$^{\ddag}$ & &.620 & .806 & .713 \\
        & T5-large & v &\textbf{.815} & .971 & .893\\ 
        & \ourmodel$_{\text{+ContractNLI}}$ & v & .813 & \textbf{.978} & \textbf{.895}\\
     \midrule
    % \multicolumn{3}{l}{\underline{\textit{zero-shot:}}} \\
    \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\textit{0-shot}}}} 
        &T5$_{\text{MNLI}}$ & v &.616 & .882 & .749 \\
        & T5$_{\text{*NLI}}$ & v &.616 & .869& .742 \\
        & \ourmodel & v & \textbf{.661} &\textbf{.904} & \textbf{.782} \\ 
     \bottomrule
    \end{tabular}
    \vspace{-5pt}
    \caption{ContractNLI results with Oracle evidence spans (excluding neutral examples). Sentence-pair models (S.P.), even in zero-shot setting, outperform the SpanNLI model that was trained on long inputs. $^{\ddag}$Results from \citet{koreeda-manning-2021-contractnli-dataset}.}
    \label{tab:contnli_oracle}
    \vspace{-4pt}
\end{table}

As its name suggests, the examples of the ContractNLI dataset are real contracts collected online. The hypotheses present different assumptions about the content of the contract. This domain is different from the one used for training our models and might present different linguistic characteristics. Therefore, we start by evaluating the NLI performance of our models in a controlled experiment using the oracle spans from the document. 

In Table~\ref{tab:contnli_oracle}, we compare our sentence-pair models, with and without training on ContractNLI, against the SpanNLI model~\citep{koreeda-manning-2021-contractnli-dataset}. SpanNLI was trained with a joint objective for both selecting the evidence spans from the document and making the NLI prediction per hypothesis. The oracle setting disentangles the NLI task from the span selection as the models are provided with the human-selected spans.

Surprisingly, we find our zero-shot sentence-pair NLI models, which were trained on a different domain, outperform the supervised SpanNLI model. \ourmodel , which was trained on all five NLI datasets performs the best, demonstrating strong NLI capabilities. We also train supervised sentence-pair NLI models using the training data from ContractNLI. To collect neutral evidence for training hypotheses with this label, we randomly select a span from the document. As expected, the sentence-pair supervised models outperform the zero-shot models, where the best model is trained over the five NLI datasets in addition to ContractNLI.
Overall, this demonstrates the superiority of the sentence-pair setting over joint objective models.


\subsection{NLI vs.\ similarity-based retrieval}
Given the promising NLI performance of sentence-pair models, we now turn to the task of identifying the relevant evidence per hypothesis in order to devise the full pipeline.
Our retrieval procedure is based on the same sentence-pair NLI models and uses the $p_e$ and $p_c$ scores of each document span against the hypothesis. We argue that if the model can successfully distinguish neutral from informative relations, we can use these scores for both retrieval and classification. Indeed, we find \ourmodel's NLI scores to provide very strong retrieval signal. 
\ourmodel ranks one of the annotated spans as the top-1 span 61\% of the time. A random baseline, in comparison, achieves less than 1\%.
% Compared to a random baseline of less than 1\%, the top-ranked span by \ourmodel's NLI scores is one of the human-annotated spans 61\% of the time.

We also experiment with similarity-based retrievers that rank the spans by the cosine similarity with the hypothesis using TF-IDF vectors~\citep{koreeda-manning-2021-contractnli-dataset}, BERT large embeddings~\citep{devlin-etal-2019-bert}, or SentenceT5 embeddings~\citep{ni2021sentencet5}. Table~\ref{tab:contnli_res} shows the precision at recall 0.8 for these zero-shot retrievers. NLI-based retrieval outperforms the similarity-based methods. Intuitively, this can be explained by the fact that two \emph{neutral} sentences can be very similar according to many measures, but uninformative for our purpose. (e.g., consider $\prem=$``$\textit{We discuss } \hyp \textit{ later}$''). Table~\ref{tab:contract_ret_examples} shows an example of such case.

\subsection{Retrieve-and-classify over documents} \label{sec:ret-and-cls}
We are now equipped to perform both evidence retrieval and classification with the same sentence-pair NLI model. First, we compute the pairwise $p_{y,i}$ scores for $\hyp$ against each span $S_i$. 
We define two methods for constructing the final prediction:
% To construct a final prediction, we define the following two methods:

\paragraph{Retrieve-and-Predict.} We aggregate over all spans by $\bar{p_y} = \max_{i}{(p_{y,i})}$, and then predict by the highest NLI score: 
% \vspace{-.5em}
\begin{equation*}
\begin{small}
\text{prediction} =
\left\{
	\begin{array}{ll}
		\argmax{(\bar{p_e},\bar{p_c})}  & \mbox{if } \max{(\bar{p_e},\bar{p_c})} > T,  \\
		\text{'neutral'} & \mbox{otherwise.}
	\end{array}
\right.
\end{small}
% \vspace{-.5em}
\end{equation*}
We simply set $T=0.5$ for the zero-shot setting, but it can be potentially tuned. Effectively, the prediction is determined by the span with the strongest sentiment towards the hypothesis.

\paragraph{Retrieve-and-Rerank.} For non-neutral predictions, we rerun the same NLI model with the top-K ranked spans retrieved for 'e' and 'c' relations. For symmetry, we do this twice, concatenating the two spans in both orders, and average the scores. Figure~\ref{fig:rerank} illustrates this process with $K=1$.

The reranking method allows the NLI model to directly contrast the span that is most entailing with the span that is most contradicting the hypothesis. 
The resultant multi-sentence premise is longer than \ourmodel's training distribution. Motivated by our earlier findings (\S\ref{sec:docnli_by_len}), we expect the model to generalize to this slightly longer but focused premise.
% This focused comparison creates a short two-sentence premise that is still relatively close to the training distribution of sentence-pair models.

% results with rerank, and compared to SpanNLI
\paragraph{Results.}
Table~\ref{tab:contnli_res} shows the main results on ContractNLI comparing sentence-pair zero-shot models with supervised ones. Surprisingly, the zero-shot sentence-pair models are competitive with the supervised SpanNLI model, even outperforming them in $F_1$(C). The supervised sentence-pair model trained on all five NLI datasets and ContractNLI performs best overall. Its retrieval performance still lacks behind SpanNLI, possibly due to only sampling random spans for neutral examples.
% the random sampling of neutral spans that doesn't utilize the full document.

% The rerank approach provides an average increase of $0.1$ $F_1$ points over the naive aggregation with zero-shot \ourmodel.
Reranking significantly improves the performance of zero-shot \ourmodel, increasing the average score by up to 27\%. We observe better performance with larger context ($K=5$).  For the supervised \ourmodel model, reranking provides only marginal gains, and increasing the context is not beneficial.

% back to DocNLI results
Returning to the DocNLI dataset, we test if our sentence-pair method can improve the low performance over long premises (\S\ref{sec:docnli_by_len}). We focus on examples with a short hypothesis (up to 20 tokens) and long premise (more than 512 tokens). Naively applying \ourmodel on these cases without sentence splitting leads to a low $0.21$ $F_1$ score. Using our retrieve-and-predict approach, the score increases up to $0.41$. Reranking doesn't seem to improve in this case, possibly due to the two-way classification format of that dataset.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/nli_rerank_2.pdf}
      \vspace{-8pt}
    \caption[]{NLI-based retrieve-and-rerank pipeline.}
      \vspace{-5pt}
    \label{fig:rerank}
\end{figure}


\begin{table}[t]
\small
    \centering
        \resizebox{\linewidth}{!}{
    \begin{tabular}{l|c|c|ccc}
    \toprule
    Model & S.P. & P@R.8 & $F_1$(C) & $F_1$(E) & AVG \\
    \midrule
    Majority vote$^{\ddag}$ &  &  - & .083 & .428 & .256 \\
    \midrule
    \multicolumn{3}{l}{\underline{\textit{supervised:}}} \\
        SpanNLI-base$^{\ddag}$ & & .663 & .287 & .765 & .526\\
        SpanNLI-large$^{\ddag}$ & & \textbf{.793} & .357 & \textbf{.834} & .595 \\
        T5-large & v & .575 & .512 & .691 & .601\\ 
        % $\quad$ + rerank & v & - & .519 & .699 \\
        \ourmodel$_{\text{+Cont.NLI}}$ & v & .580 & .521 & .754 & .637\\
        \ + Rerank$_{(K=1)}$ & v  & " & \textbf{.537}  & .741 & \textbf{.639}\\
        \ + Rerank$_{(K=5)}$ & v & " & .520 & .719 & .619 \\
     \midrule
    \multicolumn{3}{l}{\underline{\textit{zero-shot:}}} \\
        TF-IDF$^{\ddag}$ & v & .057 & - & - & -\\
        BERT emb. & v & .083& - & - & - \\
        SentenceT5 & v & .311& - & - & - \\
        T5$_{\text{MNLI}}$ & v & .397 & .261 & .551 & .406 \\
        % $\quad$ + rerank & v & - & .350 & .639 & .494\\
         T5$_{\text{*NLI}}$ & v & .397 & .247 & .594 & .420 \\
        %  $\quad$ + rerank & v & - & .341 & .656 & .499\\
         \ourmodel & v & \textbf{.412} & .257 & .573 & .415 \\ 
         \ + Rerank$_{(K=1)}$ & v & " & .363 & \textbf{.659} & .511 \\
         \ + Rerank$_{(K=5)}$ & v & " & \textbf{.404} & .652 & \textbf{.528} \\
     \bottomrule
    \end{tabular}
    }%
    \vspace{-5pt}
    \caption{Evidence retrieval and classification results of both supervised and zero-shot models on ContractNLI test set. Within sentence-pair (S.P.) models, NLI-based retrieval is more precise than similarity retrievers. Supervised S.P.\ models  outperform the joint SpanNLI model in the final classification task thanks to better $F_1$(C). $^{\ddag}$Results from \citet{koreeda-manning-2021-contractnli-dataset}.}
    \label{tab:contnli_res}
    \vspace{-8pt}
\end{table}

% \subsection{Multi-sentence hypotheses}
% \tal{possibly include SummaC here}

==> Cluster NLI paper - revised/sections/intro.tex <==
\section{Introduction}\label{sec:intro}




Natural Language Inference (NLI) involves automatically determining whether the meaning of one piece of text (i.e., hypothesis) can be inferred from another (i.e., the premise) \citep{dagan2006}. 
This formulation is relatively simple, enabling large-scale data annotation~\citep[e.g.,][]{bowman-etal-2015-large, williams-etal-2018-broad}, yet imposes complex semantic reasoning challenges (e.g., background knowledge, commonsense), leading to a useful training and evaluation NLP framework~\citep{mishra-etal-2021-looking, Sainz2022textual, vu-etal-2021-strata}.
% \looseness=-1

% The simple formulation of this task enables the collection of large datasets~\cite[][etc.]{bowman-etal-2015-large, williams-etal-2018-broad}. Also, the potentially complex semantic reasoning challenges of NLI---involving background knowledge and commonsense---make it a desirable training and evaluation framework for many NLP systems~\cite{vu-etal-2021-strata}.

% \tal{maybe short par on hyp-only bias and ANLI/ VitaminC to avoid it}
% Here, we take sentence-pair NLI models to new extents that 

%  While multiple studies have pointed out annotation artifacts in NLI and fact verification datasets that prevent trained models from generalizing~\citep{gururangan-etal-2018-annotation,mccoy-etal-2019-right,poliak-etal-2018-hypothesis, schuster-etal-2019-towards}, new curated datasets were shown to support better  robustness~\citep{nie-etal-2020-adversarial,schuster-etal-2021-get}.

% par on hyp-only bias and recent datasets that show promising capabilities
% yet challenging to NLP systems. 
% makes it relatively straightforward to humans, enabling
% Being a semantic task that is relatively easy for humans, and 



Formally, in NLI, we are interested in learning a function $\func: (\hyp \times \prem) \rightarrow \mathcal{Y}$ that predicts the relation $Y$ between the provided premise $\prem$ and the examined hypothesis $\hyp$, where $\mathcal{Y} = \{\mathrm{entailment, neutral, contradiction}\}$.\footnote{This formulation also fits the task of fact-checking a claim against given evidence~\citep{thorne-etal-2018-fever}, therefore henceforth we use the NLI terminology for both tasks.}
In most NLI datasets, $\hyp$ and $\prem$ are short texts consisting of one or few sentences, allowing current Large Language Models (LLMs) with limited input length to process the two with cross-attention. In practice, however, many systems require operating over long texts such as full documents or even collections of documents without knowing a priori which parts are most relevant.

Consider the example in Figure~\ref{fig:intro}. The system is trying to reason over a collection of documents and find statements that they all agree upon (consesnus), or alternatively, find potential disagreements across documents. Instead of having a clear hypothesis-premise pair, each statement across all documents is an hypothesis of interest that should be evaluated against all other documents as the premise.


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/cluster_nli.pdf}
                   \vspace{-5pt}
    \caption[]{Illustration of our procedure for flagging potential discrepancies in document clusters (\S\ref{sec:clusters_method}). This is a real-world example from Wikipedia's translated articles in different languages about the novel Dracula (as of Feb.\ 2022).\footnotemark\ Our model identified the French Wikipedia to disagree with other articles on the nationality of the author.}
    \label{fig:intro}
                       \vspace{-8pt}
\end{figure*}

In this paper, we focus on these realistic scenarios and present retrieve-and-classify methods for inferring over long and out-of-distribution (OOD) inputs in a zero-shot fashion. As this setting emphasizes the need for a robust sentence-pair NLI model as a backbone, we train on multiple datasets, including adversarial and contrastive ones~\citep{nie-etal-2020-adversarial,schuster-etal-2021-get} to increase the model's robustness and avoid dataset-specific biases~\citep{gururangan-etal-2018-annotation,mccoy-etal-2019-right,poliak-etal-2018-hypothesis, schuster-etal-2019-towards}.

% % we train a NLI model on multiple sentence-pair datasets and develop zero-shot aggregation methods for supporting longer and out-of-distribution (OOD) inputs. Our pipeline relies on 

% While multiple studies have identified certain dataset-specific biases in NLI-trained models~\citep{gururangan-etal-2018-annotation,mccoy-etal-2019-right,poliak-etal-2018-hypothesis, schuster-etal-2019-towards}, new curated datasets were shown to support better  robustness~\citep{nie-etal-2020-adversarial,schuster-etal-2021-get}. Our OOD and real-world applications test this to new extents 

Our proposed pipelines go beyond the length and format supported by most LMs and include new retrieval, aggregation and classification solutions---all based on the same classifier. Thereby, we continue the line of work on evaluating the robustness of such models and their ability to truly capture semantic relations. Moreover, long inputs highlight the commonly overlooked yet practically important challenge of specifying ``neutral'' relations. For example, mistaking certain part of the premise as entailing instead of neutral can overshadow another segment that contradicts the hypothesis.




We first evaluate the zero-shot performance of our multi-task NLI model on $\prem$s that are longer than the examples seen in training, but short enough to allow supervised LMs with similar length constraints to perform well~\citep{yin-etal-2021-docnli}. In the zero-shot setting, we find that models generalize beyond the training distribution, but drop in performance for very long $\prem$s ($>400$ tokens).
% \tal{complete after DocNLI length experiments}


% \footnotetext{\href{https://fr.wikipedia.org/w/index.php?title=Dracula&oldid=190970820}{fr.wikipedia.org/w/index.php?title=Dracula\&oldid=190970820}}

\footnotetext{\url{https://fr.wikipedia.org/w/index.php?title=Dracula&oldid=190970820}}

Then, we turn to focus on the scenario of having a full document as $\prem$~\citep{koreeda-manning-2021-contractnli-dataset}. A typical approach---the default behavior of most LMs---would truncate the end of the document beyond some predefined length (e.g., 512 tokens). However, this might remove and ignore important information.
% , and still carry very long inputs, beyond the training distribution.
Instead, we hypothesize that a good NLI model should be able to separate the wheat from the chaff and distinguish neutral spans towards $\hyp$ from informative ones. To this end, we develop a solely NLI-based retrieve-and-classify approach that outperforms similarity-based retrievers and whole-document classifiers.

Finally, we go further and demonstrate the utility of our model for reasoning over entire clusters of related documents. Our proposed procedure, illustrated in Figure~\ref{fig:intro}, ranks all of the cluster's spans by their entailment relations with spans from other documents. Testing our approach on Wikipedia introductions on the same topic in different languages, we successfully identify claims that are unique to one version and contradicted by others.

In summary, this work stretches sentence-pair NLI models to new practical capabilities and demonstrates their direct utility in real-world applications.  
%
Our main contributions include: \vspace{-0.5em}
\begin{itemize}[leftmargin=*]
    \item A multi-task sentence-level NLI model with strong zero-shot and supervised performance for both evidence retrieval and classification. \vspace{-0.5em}
    \item Simple and effective retrieve-and-classify methods to extend sentence-pair semantic classifiers and outperform  whole-document models.\vspace{-0.5em}
    % \item An analysis of similarity-based retrieval versus NLI-based retrieval for entailment prediction, highlighting the necessity of the latter. \vspace{-0.3em}
    \item A new entailment task and dataset that requires inference over clusters of documents (\S\ref{sec:wiki_clusters}).\footnote{We intend to release this new dataset upon publication.} \vspace{-0.5em}
    \item Demonstrating the utility of our approach to reveal real and simulated discrepancies in Wikipedia pages by automatically comparing with content from multiple translated articles.
\end{itemize}



==> Cluster NLI paper - revised/sections/long_inputs.tex <==
\section{Long and OOD Inputs}\label{sec:docnli}



\begin{table}[t]
\small
    \centering
    \begin{tabular}{l|cc}
    \toprule
    Model & Dev. & Test \\
    \midrule
    Random & .198 & .199 \\
    \midrule
    \multicolumn{3}{l}{\underline{\textit{supervised:}}} \\
    Longformer-base$^*$~\citep{yin-etal-2021-docnli} & .462 & .444  \\
     Roberta-large~\citep{yin-etal-2021-docnli} & .631 & .613  \\
     T5-large & .642 &.618 \\
     \midrule
    \multicolumn{3}{l}{\underline{\textit{zero-shot:}}} \\
     \ourmodel & .341 & .345 \\     
     \ourmodel$_{\text{tuned}}$ & .409  & .408 \\  
     \bottomrule
    \end{tabular}
                   \vspace{-5pt}
    \caption{$F_1$(E) scores on the \textsc{DocNLI}(-ANLI) binary classification dataset. The zero-shot shot predictions are based on a threshold $T$ on the entailment score which is either set to $0.5$ or \emph{tuned} over $0.2\%$ of the dev set. $^*$Longformer's scores are over the full DocNLI.}
    \label{tab:res_docnli}
    \vspace{-8pt}
\end{table}


We start by exploring the use of \ourmodel on examples that differ from the training data in both length and domain. We hypothesis that a robust semantic reasoning model trained on top of a large LM that memorized world knowledge, should achieve competitive results even when applied to a new domain without any finetuning (i.e., zero-shot). 

For this experimentation, we use the DocNLI dataset~\citep{yin-etal-2021-docnli} and remove ANLI from it since ANLI was included in our training data.\footnote{The ANLI examples cover only 1.2\% of the DocNLI test set, so the difference is minimal. \ourmodel and \ourmodel$_{\text{tuned}}$ get .350 and .410 $F_1$ scores on the full test set, respectively. } 
A large portion of DocNLI is based on news articles where the hypothesis is a short summary of an article and the premise is the article itself. 

DocNLI uses only two classes, ``entail'' vs.\ ``not entail'', by merging the ``neutral'' and ``contradiction'' definitions. We discuss different zero-shot aggregation techniques from 3-way models to binary classification in Appendix~\ref{sec:binary_aggr}.
The ``not entail'' instances are created with both rule-based and LM-based local perturbations techniques over the positive pairs. This results in a slightly different task definition than NLI since in practice even altered (i.e., ``fake'') texts can still factually agree with the hypothesis~\citep{schuster-etal-2020-limitations}. \citet{yin-etal-2021-docnli} account for this discrepancy by augmenting the training set, but zero-shot NLI models might be affected by this provenance-based rather than factual-based partition of the test set.
%


% adapting to 2-way classification





\subsection{Out-of-the-box adoption}
\citet{yin-etal-2021-docnli} found a model with an input limit of 512 tokens to perform well on DocNLI, by simply truncating the remainder of the input.
% , suggesting that the relevant information for prediction mostly appears at the beginning of the premise. 
We follow their setting and evaluate a naive zero-shot application of \ourmodel on this new domain. Table~\ref{tab:res_docnli} shows that \ourmodel performs much better than a random baseline and is competitive with some of the supervised models, indicating promising transfer potential.
% This suggests that \ourmodel is basing its predictions on features that are general enough to transfer to new domains and settings.

\subsection{Performance by input length} \label{sec:docnli_by_len}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.46\textwidth]{figures/docnli_by_length.png}
        \vspace{-4pt}
    \caption[]{Effect of input length of DocNLI examples on naive applications of \ourmodel (zero-shot, without sentence splitting). The blue line shows $F_1$ score as a function of hypothesis length ($|\hyp|$). The orange line bins examples by the premise length ($|\prem|$), focusing only on short hypotheses (where $|\hyp|\le20$). For short hypotheses, the performance stays high even beyond the training distribution, but sharply drops around the input length limit of the model.}
    \label{fig:docnli_by_len}
     \vspace{-5pt}
\end{figure}

Figure~\ref{fig:docnli_by_len} shows the $F_1$ score of \ourmodel as a function of the input length. 
Our first observation is that the performance is highly affected by the length of the hypothesis. \citet{yin-etal-2021-docnli} observed a similar trend even with supervised models. We conjecture that this is due to the natural increase in ambiguity with the hypothesis' length, as it is more likely to contain multiple atomic facts and it's unclear which is the one in question. This motivates our inference pipelines in the following sections that focus on concise hypotheses and aggregate when needed.

Second, we look at the performance as a function of the premise length. To focus on examples where the hypothesis is well defined, we only consider cases with a short hypothesis of no more than 20 tokens (total of 5,932 cases from DocNLI(-ANLI) test set). As the orange line in Figure~\ref{fig:docnli_by_len} shows, \ourmodel performs well on these cases even when the premise is much longer than the inputs that the model was trained on, demonstrating promising potential for zero-shot applications. However, the performance significantly drops when reaching the input length limit, requiring to truncate the premise. Next, we discuss methods for retrieving and aggregating predictions of sentence-pair models over long documents.

% Second, we see that the performance gradually decreases with the total input length, though remains better than random even beyond the model's input limit. This aligns with the earlier observation that in many of the dataset examples the crucial information is at the beginning of the premise. Yet, in some long inputs the model might be missing important information.

% \subsection{Breaking down long premises}
% To address the premise length limitation with a zero-shot NLI model, we split each long premise into multiple sentences, evaluate the hypothesis against each of them independently, and aggregate the scores by taking the max $p_y$ across sentences. To evaluate this approach, we collect examples with a short hypothesis ($<20$ tokens) and long premise (combined length over 512 tokens) from the test set. Without splitting, \ourmodel's $F_1$ score on this subset is only $0.228$, only slightly above random.

% Following the splitting and aggregation approach, predicting with 'c' threshold achieves $0.333$ $F_1$ with $T=0.5$, and up to $0.412$ with $T=0.2$. In this setting, 'e' threshold reaches only $0.239$ $F_1$.

% more expensive but can be run in parallel, unlike models that process very long inputs and have to run self-attention on long input.

% Instead, we aggregate the predictions per hypothesis by taking the maximum $p_y$ across all predictions against each of the premise sentences.


==> Cluster NLI paper - revised/sections/model.tex <==
\section{Model and Definitions}\label{sec:model}
% In this section we describe the training process of our main model, and how we use it to obtain prediction scores

Our pipelines build on entailment scores for hypothesis-premise pairs.
To predict these scores, we train a sentence-pair NLI model that we use as the backbone for all methods. Specifically, we pick the T5 encoder-decoder architecture as it has been shown to perform well in multi-task and transfer settings~\citep{arib2021ext5, t5_paper}.
See Appendix~\ref{sec:technical_det} for more technical details.

% output space (normalizing over three outputs)
\newpar{Definitions.}
As T5 is a seq-to-seq model, we train it over the training set $(\hyp, \prem, Y) \sim \mathcal{D}_{\mathrm{train}}$ by feeding the following format to the encoder:
``\emph{entailment: $\hyp$ [SEP] $\prem$}.'' The decoder's goal is to generate a single character 'e', 'n', or 'c', representing 
the three classes in $\mathcal{Y}$: entailment, neutral, and contradiction, respectively. Thereafter, when making a prediction on a new pair $(\hyp, \prem) \in \mathcal{D}_{\mathrm{test}}$, we encode the input and measure the decoder's score $s_y$ for each of the three classes. Finally, we normalize the three scores with a softmax operator: $p_y=\softmax(s_e, s_n, s_c)[y]$. Note that  these scores should not be directly treated as class probabilities as they are not calibrated, especially when evaluating out-of-domain inputs. However, as we will show in our experiments, they can be readily tuned or leveraged as a valuable signal for textual semantic relations.

% to generate a prediction for the relation of the input sentence pair. Given an input $x_{\text{h}}$


\newpar{The \ourmodel model.}
To train our model, we use the following sentence-pair datasets: 
 SNLI~\citep{bowman-etal-2015-large}, MNLI~\citep{williams-etal-2018-broad}, ANLI~\citep{nie-etal-2020-adversarial}, FEVER~\citep{thorne-etal-2018-fever}, and VitaminC~\citep{schuster-etal-2021-get}. For FEVER, we use the sentence-pair version from VitaminC with retrieved evidence to neutral claims.
 
 
% \begin{itemize}
%     \item SNLI~\citep{bowman-etal-2015-large}: \tal{todo}
%     \item MNLI~\citep{williams-etal-2018-broad}: 
%     \item ANLI~\citep{nie-etal-2020-adversarial}:
%     \item FEVER~\citep{thorne-etal-2018-fever}: Neutral cases of FEVER, evidence sentences are randomly picked from the retrieved article for each claim by a BM25 retrieval. 
%     \item VitaminC~\citep{schuster-etal-2021-get}:
% \end{itemize}
This multi-task training is important for improving the robustness of the model by leveraging a large amount of diverse data. Also, including adversarial (ANLI) and contrastive (VitaminC) examples was shown to prevent the model from relying on hypothesis-only biases. Table~\ref{tab:train_datasets} shows the input length statistics of the datasets according to the English sentence-piece tokenizer of T5. 
%Being sentence-pair examples, the input lengths are far below the common input length limit of 512 tokens. 
% Yet, the conciseness of the input makes the NLI task less ambiguous as the context is generally more focused.
Having concise and short inputs generally makes the task less ambiguous---as claim in question is clear---and focused on the textual entailment component.

We denote our T5 mutli-task NLI model trained on all 5 datasets \ourmodel. Our application-specific pipelines will differ in the way that they make use of \ourmodel's predictions. 
We also experiment with models trained only on MNLI without multi-tasking (-M.T), only on the three *NLI datasets (-F.V), or with ContractNLI~\citep{koreeda-manning-2021-contractnli-dataset} examples.


% datasts statistics


% TODO: define inference against full doc.

% define probability of each class

\begin{table}[t]
\small
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|zzc}
\toprule
        Train dataset & \multicolumn{1}{c}{Hypothesis length} & \multicolumn{1}{c}{Premise length} & \multicolumn{1}{c}{Train pairs}   \\
        \midrule
        MNLI & 13.23 (7-20) & 27.57 (9-50) & 392,702 \\
        SNLI & 9.50 (5-15) & 16.86 (9-27) & 550,152\\
        ANLI & 13.32 (7-21) & 79.95 (53-111) & 162,865\\
        FEVER & 12.50 (8-18) & 47.98 (21-82) & 178,059\\
        VitaminC & 18.18 (10-29) & 43.03 (19-72) & 370,653 \\
    \bottomrule
    \end{tabular}
        }%
                       \vspace{-5pt}
    \caption{Training datasets of \ourmodel. We report the average length of the tokenized (for T5) hypothesis and premise, and the 10th-90th percentiles in parentheses.}
    \label{tab:train_datasets}
      \vspace{-10pt}
\end{table}




==> Cluster NLI paper - revised/sections/related.tex <==
\section{Related Work}\label{sec:related}
As mentioned in the introduction, the NLI task~\citep{dagan2006, dagan2013recognizing}, sometimes called Recognizing Textual Entailment (RTE), was extensively studied by the NLP community over the past several years as a semantic reasoning benchmark~\cite[see][for surveys]{poliak-2020-survey, storks2019recent}. The field of fact verification~\citep{vlachos-riedel-2014-fact} also recently gained increased attention~\citep{Bekoulis, kotonya-toni-2020-explainable, Guo2022ASO, zeng2021automated}, sharing similar pair-wise semantic inference challenges, together with evidence retrieval.
While both tasks were found to be vulnerable to idiosyncrasies~\citep{gururangan-etal-2018-annotation,mccoy-etal-2019-right,poliak-etal-2018-hypothesis, schuster-etal-2019-towards}, methods and datasets for reducing the bias were proposed~\citep{belinkov2019, karimi-mahabadi-etal-2020-end, Shah_Schuster_Barzilay_2020, utama-etal-2020-towards, utama-etal-2021-avoiding, Yuxiang2022}.
% Our work continues this research direction by testing the robustness of multi-task NLI models in clusters-level inference.


% NLI modeling (sentence embedding vs. cross-attention)

% bias in nli and mitigation

% Use for real applications (summarization/ dialog/ automatic editing)
Recently, NLI-style models were expanded for concrete purposes beyond benchmarking. For example, showing promising potential in verifying the factual correctness of dialog~\citep{gupta2021dialfact, honovich-etal-2021-q2}, summarization~\citep{chen-etal-2021-improving, eyal-etal-2019-question, alex2021qafacteval, SummaC}, and QA~\citep{bulian2022tomayto, chen-etal-2021-nli-models, mishra-etal-2021-looking} systems.
The NLI format was also found helpful for general self-training~\citep{vu-etal-2021-strata}. 
Here, we focus on real-world direct applications such as automatic contract analysis~\citep{koreeda-manning-2021-contractnli-dataset} and identifying discrepancies in document collections.

In parallel work, \citet{utama-etal-2022-falsesum} improve NLI models for evaluating summaries by generating in-domain data with automatic perturbations to simulate contradictions. We observe similar improvements when training the backbone NLI models on in-domain data for ContractNLI (supervised vs.\ zero-shot setting). Any additional improvements to the NLI model, aimed towards the target domain, are likely to further improve the reasoning capabilities of the retrieve-and-classify pipeline.



% edit modeling (FRUIT)
% zzz
% Our discrepancy finding experiments (\S\ref{sec:res_wiki}) also relate to recent work on fact-checking in-the-wild, without having a specific claim structure~\citep{park2021faviq, thorne2021evidence}. However, unlike previous work that depend on user queries, we seek for claims that stand out in collections of related documents. Focusing on Wikipedia, our discrepancy flagging is also complementary to other moderation-assisting research such as evidence-supported edit suggestions~\citep{iv2021fruit, schuster-etal-2021-get, Shah_Schuster_Barzilay_2020}. 


% Uncertain Natural Language Inference (Chen et al., ACL 2020)

==> sections/app_summac.tex <==
\section{Multi-sentence hypotheses} \label{sec:summac}

Recently, \citet{SummaC} presented the \summac benchmark for predicting the factual consistency of summaries with their source. The benchmark includes the following six datasets: CGS~\citep{falke-etal-2019-ranking},
XSF~\citep{maynez-etal-2020-faithfulness},
Polytope~\citep{huang-etal-2020-achieved},
FactCC~\citep{kryscinski-etal-2020-evaluating},
SummEval~\citep{fabbri-etal-2021-summeval},
FRANK~\citep{pagnoni-etal-2021-understanding}.
We follow the zero-shot setting here as our main focus on this paper is zero-shot applications of NLI models. For fair comparison with the zero-shot setting of \citet{SummaC}, however, we also tune the threshold on the validation set for each dataset, and report the results on the test set. In early exploration we found naive threshold settings to be competitive as well.

Their proposed zero-shot solution is similar to our approach, relying on multi-task sentence-pair NLI models and aggregating the predictions. Their method, however, aims to achieve a single score for the whole summary. Instead, we focus on short hypotheses and on identifying and flagging specific spans that stand out in a collection of related documents. For completeness, we evaluate our \ourmodel model on this benchmark and also experiment the reranking approach for this application.

Specifically, the \summac zero-shot method ($\summac_{\mathrm{ZS}}$) computes the NLI score of each sentence from the summary with each sentence in the document. Then, the final ``factual consistency'' score for the summary is the average over the maximum entailment score ($p_e$) for each sentence of the hypothesis.

To account for the hypothesis aggregation step, we had to slightly adjust our reranking approach. Specifically, we experiment with the following settings:
\begin{itemize}[leftmargin=*]
    \item \textbf{\ourmodel:} We simply replace the backbone NLI model of $\summac_{\mathrm{ZS}}$ with \ourmodel and follow the same aggregation process (without reranking). Hence, the main difference is that we use T5-large~\citep{t5_paper} instead of BERT-large~\citep{devlin-etal-2019-bert}, and possible other small differences regarding the training configuration.
    \item \textbf{+ soft rerank:} For each of the hypothesis sentences, the entailment score is recomputed by running \ourmodel again with both the most supporting and the most contradicting sentences from the document, according to the first-pass NLI scores. Since there is already a $\max$ operation over the scores, this can be viewed as smoothing the score by adding the most contradicting sentence to the context.
    \item \textbf{+ hard rerank:} We perform the following two modifications over the soft method: (1) we use the difference between entailment and contradiction scores from the rerank run ($p_e - p_c$); and (2)
    we set a $\min$ instead of $\mathrm{mean}$ operation, effectively requiring \emph{all sentences} of the hypothesis to be supported.
\end{itemize}


The results are summarized in Table~\ref{tab:summac}. Replacing the backbone model with ours improves the overall performance by absolute $1.2$ points. This overall improvement comes despite a drop of almost 10 points on the Polytope dataset. We note that the ``factual consistency'' definitions used for \summac label summaries with ``addition'' (of unnecessary content) or ``omission'' errors as negative. These errors related more to the quality of the summary rather to its correctness. Therefore, we do not expect zero-shot NLI models to them. 

The effectiveness of reranking varies by dataset. The best overall performance is achieved with hard reranking, improving over the previous aggregation in 4 out of the 6 datasets, and obtaining an overall gain of $0.2$ points.


\begin{table*}[t]
\small
    \centering
    \begin{tabular}{l|dddddd|d}
    \toprule
    Method & \multicolumn{1}{c}{CGS} & \multicolumn{1}{c}{XSF} & \multicolumn{1}{c}{Polytope}& \multicolumn{1}{c}{FactCC} & \multicolumn{1}{c}{SummEval}& \multicolumn{1}{c}{FRANK} & \multicolumn{1}{c}{Overall}\\
    % \cmidrule{2-4}
    \midrule
    $\summac_{\mathrm{ZS}}$ & 70.4 & 58.4 & \textbf{62}.\textbf{0} & 83.8 & 78.7 & 79.0 & 72.1 \\
    \midrule
    \ourmodel & 79.3 & 59.3 & 52.4 & \textbf{89}.\textbf{5} & 77.2 & \textbf{82}.\textbf{1} & 73.3 \\
    + soft rerank & 79.6 & 62.7 & 52.8 & 86.1 & 78.5 & 80.4 & 73.3 \\
    + hard rerank & \textbf{80}.\textbf{5} & \textbf{64}.\textbf{2} & 55.1 & 83.3 & \textbf{79}.\textbf{7} & 78.4 & \textbf{73}.\textbf{5} \\ 
     \bottomrule
    \end{tabular}
    \caption{Balanced accuracy of zero-shot methods on the \summac benchmark.}
    \label{tab:summac}
\end{table*}

==> sections/clusters.tex <==
\section{Analyzing Document Clusters}\label{sec:clusters}
So far, we dealt with evaluating a single, short or long hypothesis against a long premise. In some applications, however, the user might not know which hypothesis to check, but rather would like to query over their corpus to identify the most extreme ones. 
% For example, in the news domain we commonly have a collection of articles written by different sources and describing the same event. 
For example, consider a collection of news articles on the same topic written by different sources.
Typical questions to ask about this corpus could be: \emph{``is there any claim made by one article that other articles disagree with?''}, or other aggregations like \emph{``what is the most controversial claim?''} or \emph{``is there consensus on some claims in the corpus?''}

Answering such questions goes beyond the typical NLI setting and requires understanding a complex many-to-many relation between the documents, involving multiple alignment and reasoning challenges. Therefore, any solution with low signal-to-noise rate is likely to fail. Following our promising findings on the robustness of \ourmodel, we rely on it to construct a cluster-level algorithm for answering these queries. 

To test this setting, we create a dataset with clusters of popular Wikipedia articles on the same topic written in different languages, translated to English. Each version of Wikipedia is managed by a different community, leading to occasional disagreements or mistakes~\citep{unified_wiki}, or even the risk of version-specific conspiracy theories.\footnote{\url{www.bbc.com/news/technology-59325128}} We would like to create a system that can scan these articles and find discrepancies, potentially flagging instances to be checked by content moderators.

\subsection{Wikipedia clusters evaluation dataset}\label{sec:wiki_clusters}
We create clusters of introductions to popular Wikpedia articles about the same topic but written by different communities in multiple (up to 11) languages. 
To simplify the setting, we translate all introductions to English with Google Translate API. See App.~\ref{sec:wikiclusters_details} for more details.

For each cluster, we are interested in identifying claims that appear in at least one article and disagree with most other articles. To this end, we examine two settings:

\paragraph{Corrupted articles.}
We synthetically corrupt the English version of each article by inserting a local edit to one of the sentences. The task is to use the other articles of that cluster to identify the sentence that was changed. While it is possible that all other articles don't mention any information about the specific corrupted fact, thanks to the popularity of the chosen articles and languages we find that mostly at least one of the articles includes sufficient information to refute the corrupted sentence. 

To create the corruptions, we use the edits from the test set of the VitaminC dataset~\citep{schuster-etal-2021-get} that express opposite relations towards a mutual claim. 
In total, we create 824 instances based on 144 different topics. In each instance, we corrupt a single sentence from one of the English articles, and provide the 10 related articles from other languages to help identify which fact was changed.

We note that \ourmodel observed Wikipedia sentences (from other articles) in the training mixture. However, they were only used as the premise, whereas here they also represent the hypothesis.

\paragraph{Real discrepancies.}
We test our method in-the-wild, looking for discrepancies in current Wikipedia. Here, we search across all pages in a cluster and look for sentences that disagree with most other pages. Due to the dynamic nature of Wikipedia and since we lack annotations, we use qualitative evaluation and focus on precision of top-ranked sentences rather than recall.

% Since Wikipedia is constantly edited and updated, we use qualitative evaluation and focus on precision rather than recall.



\subsection{Identifying factual discrepancies}
Algorithm~\ref{alg:cluster} describes our approach for ranking the spans across all cluster documents according to their likelihood of being a discrepancy.\footnote{When looking for consensus, $p_c$ is replaced by $p_e$.}
Each span is compared against all other spans from all documents. The score is determined by the most contradicting pairing from each document and averaged across the cluster. While this procedure requires many calls to the NLI model (quadratic in number and size of documents), they are independent and can be easily batched and parallelized. 

\paragraph{Results.}
For our simulated article corruptions, we only rank sentences from the English articles. Table~\ref{tab:wiki_corrupt} reports the results. In addition to our main method, we tried reverse rank by entailment score, but find it to perform even worst than random. We find this to be caused by pairings that support unmodified facts in the corrupted sentence. When ranking by contradiction, \ourmodel performs the best and successfully flags 68\% of the corruptions as its top prediction.

\begin{algorithm}[t]
\small
\caption{Find factual discrepancies in a cluster.}\label{alg:cluster}
\begin{algorithmic}
\Require Cluster of documents $\mathcal{C}$ with spans $\mathcal{S}$, and NLI model.
\Ensure Sorted spans by discrepancy likelihood.
\State $\omega_{i,j} \gets 0 \quad \forall \text{ span } j \text{ in document } i$
\For{$D_i \in \mathcal{C}$}
\For{$S_j \in D_i$}
\State $\hyp \gets S_{i,j}$; $\quad \Omega \gets \{ \}$ 
\For{$D_k \in \mathcal{C} \setminus D_i$}
\State $\Gamma \gets \{ \}$ 
\For{$S_{k,l} \in D_k$}
\State $p_c \gets \text{\ourmodel}(\hyp, S_{k,l})[c]$
\State $\Gamma \gets \Gamma \cup \{p_c\}$
\EndFor
\State $ \Omega \gets \Omega \cup \max(\Gamma)$ 
\EndFor
\State $\omega_{i,j} \gets \mathrm{mean}(\Omega)$ 
% \State $\omega_{i,j} \gets \sum(\Omega)/ |\Omega|$ 
\EndFor
\EndFor
\Return $\mathcal{S}$ sorted by respective $\omega$
\end{algorithmic}
\end{algorithm}



% \paragraph{Discrepancies in-the-wild}
When applying our method on real Wikipedia articles, without any simulated edits, we don't know if there are any current discrepancies. We rank all sentences across all articles in a cluster and inspect the top spans. Surprisingly, even though we took the most popular pages and top moderated languages, our method quickly identified existing inconsistencies. See Appendix~\ref{sec:wiki_examples} for examples.

For instance, as depicted in Figure~\ref{fig:intro}, we find the French Wikipedia to disagree with other versions on the nationality of the author Bram Stoker. \ourmodel ranked this sentence highest among the 53  sentences of that cluster.
Investigating the page's history, this claim was introduced by an edit\footnote{\href{https://fr.wikipedia.org/w/index.php?title=Dracula&diff=133445656&oldid=133334932}{fr.wikipedia.org/w/index.php?title=Dracula\&\\diff=133445656\&oldid=133334932}} in Jan.\ 2017 and remained unchanged for over 5 years.

Interestingly, when looking for consensus and ranking sentences by agreement score, \ourmodel returns the related sentence from the English version that avoids stating the author's nationality: \emph{``Dracula is a novel by Bram Stoker, published in 1897.''} Intuitively, shorter statements have a higher chance of obtaining consensus.

% rank of prediction
In another example, we look at the articles about ``Big Ben''. The top discrepancy prediction was a sentence from the Chinese version that was likely mistranslated due to multiple segmentation options. While this does not necessarily reveal a mistake in the original document, it shows the potential of this approach for flagging translation mistakes when related sources are available. 
The second ranked sentence identifies a statement from the Swedish page regarding the monument's official name. Upon manual verification, even though articles discuss several names that were changed over time, none seem to directly support that claim.


\begin{table}[t]
\small
    \centering
    \begin{tabular}{l|ccc}
    \toprule
    Model & \multicolumn{3}{c}{Accuracy@K} \\
    % \cmidrule{2-4}
    & K=1 & 5 & 10 \\
    \midrule
    Random & 17.11 & 46.53 & 73.68 \\
    \midrule
     \multicolumn{4}{l}{\underline{\textit{Reversed ranking by entailment:}}} \\
    % T5$_{\text{MNLI}}$ & 3.03 & 31.92 & 68.08 \\
    %  T5$_{\text{*NLI}}$ & 8.37 & 48.30 & 76.46 \\
     \ourmodel &1.46 & 17.35 & 40.29 \\
    \midrule
     \multicolumn{4}{l}{\underline{\textit{Ranking by contradiction:}}} \\
    T5$_{\text{MNLI}}$ & 35.32 & 67.60 & 83.37 \\
     T5$_{\text{*NLI}}$ & 38.59 & 70.39 & 83.13 \\
     \ourmodel & \textbf{68.20} & \textbf{89.08} & \textbf{95.15} \\
     \bottomrule
    \end{tabular}
    \caption{Wikipedia corruption detection results by different ranking methods/ models. Accuracy of including the corrupted sentence within the top K predictions.}
    \label{tab:wiki_corrupt}
\end{table}

==> sections/full_docs.tex <==
\section{Operating Over Full Documents}\label{sec:fulldoc}

In this section, we turn our focus to applications where a specific hypothesis is evaluated against long texts. Formally, we assume that $\prem$ is a document consisting of $n$ sentences $S_{1:n}$ and we don't know which part of the document is most relevant for verifying or rejecting $\hyp$. 
% This is a common practical setting where the user is interested in knowing whether a document agrees or contradicts with a specific statement.
It is common in this case to not only ask for the truthfulness of the given statement, but to also point to the exact evidence in the document that led to this conclusion. 
% In this case, it is likely that the user will require the automated system to not only predict the relation between the statement and the document, but to also point to the exact evidence from the document that led to this conclusion. 
This is a crucial requirement as it both assists in interpreting and trusting the model (e.g., avoiding hypothesis-only bias), and can practically save time when having to manually verify the prediction.
% Interpreting the model's predictions is crucial for both efficiently verifying the output (e.g., ensuring no hypothesis-only bias~\citep{gururangan-etal-2018-annotation,poliak-etal-2018-hypothesis, schuster-etal-2019-towards}), and to assist the user in providing justifications to a third-party.

% 1. performance does go down even before we meet the limit
% 2. this hard constraint makes the model less adaptable inputs of any length
% 3. interpretability limitation
Following our observation that models can generalize beyond the length of training examples (\S\ref{sec:docnli_by_len}), one might consider simply increasing the limit during inference. However, there are several downsides to this approach. 
First, as Figure~\ref{fig:docnli_by_len} shows, the performance starts decreasing even before reaching the length limit. Second, due to the quadratic relation between the cost of the self-attention layer and the sequence length~\citep{tay2021long, attention_all_you_need}, increasing the length of the input has significant impact on memory consumption and latency. Lastly, this approach doesn't directly support the important interpretability requirement discussed above as it is unclear which part of the long document led the model to its prediction.

% breaking benefits:
% 1. flexible to any input form
% 2. aligns well with the training distribution on NLI
% 3. parallel computation
Instead, we opt to break the long document into individual sentences and make point-wise predictions against the hypothesis before aggregating them to the final prediction. This approach can readily extend to any document length without any modification to the core NLI model. Also, this way the model evaluates examples that are more aligned with the sentence-pair training distribution. While it requires $n$ inference runs of the NLI model instead of a single pass, the cost increase is linear in $n$, unlike the option of increasing the input length limit where the increase is quadratic. Also, these inference passes can be computed in parallel with batches to improve efficiency.
% , reducing the overall latency and flexibly controlling for memory usage.

This point-wise approach, however, has some limitations. First, it requires a robust sentence-pair model that can reliably separate neutral sentences from relevant ones. Second, it doesn't immediately support multi-hop inference over multiple sentences~\citep{jiang-etal-2020-hover}.  This can be partially addressed with preprocessing techniques \cite[e.g.,][]{choi-etal-2021-decontextualization}. In practice, we don't observe this limitation in our explored applications as most sentences are self-contained in these domains.
% breaking down limits
% 1. requires robust models (cleaning "neutral")
% 2. doesn't immediately support multi-hop reasoning

\paragraph{Experimental setting.}
 We use the ContractNLI dataset~\citep{koreeda-manning-2021-contractnli-dataset} as our main testbed for this part. Unlike the DocNLI data where models with limited input length were shown to perform well, simply truncating ContractNLI inputs to 512 tokens leads to random results. As the documents in ContractNLI contain 80 sentences on average, this setting presents two challenges: (1) identifying and retrieving the relevant evidence sentences per hypothesis, and (2) making the final prediction.
We will also revisit the long premises of DocNLI and show that this approach is beneficial there as well.
While we focus here on short hypotheses, in App.~\ref{sec:summac} we evaluate on \summac~\cite{SummaC} with multi-sentence hypotheses.


\subsection{ContractNLI with oracle spans}


\begin{table}[t]
\small
    \centering
    \begin{tabular}{ll|c|ccc}
    \toprule
    & Model & S.P. & $F_1$(C) & $F_1$(E) & AVG \\
    \midrule
    & Majority vote$^{\ddag}$ &  &.239 & .645 & .442  \\
    \midrule
    % \multicolumn{3}{l}{\underline{\textit{supervised:}}} \\
    \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{\textit{supervised}}}} 
        & SpanNLI-base$^{\ddag}$ & & .657 & .816 & .736 \\
        & SpanNLI-large$^{\ddag}$ & &.620 & .806 & .713 \\
        & T5-large & v &\textbf{.815} & .971 & .893\\ 
        & \ourmodel$_{\text{+ContractNLI}}$ & v & .813 & \textbf{.978} & \textbf{.895}\\
     \midrule
    % \multicolumn{3}{l}{\underline{\textit{zero-shot:}}} \\
    \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\textit{0-shot}}}} 
        &T5$_{\text{MNLI}}$ & v &.616 & .882 & .749 \\
        & T5$_{\text{*NLI}}$ & v &.616 & .869& .742 \\
        & \ourmodel & v & \textbf{.661} &\textbf{.904} & \textbf{.782} \\ 
     \bottomrule
    \end{tabular}
    \vspace{-5pt}
    \caption{ContractNLI results with Oracle evidence spans (excluding neutral examples). Sentence-pair models (S.P.), even in zero-shot setting, outperform the SpanNLI model that was trained on long inputs. $^{\ddag}$Results from \citet{koreeda-manning-2021-contractnli-dataset}.}
    \label{tab:contnli_oracle}
    \vspace{-4pt}
\end{table}

As its name suggests, the examples of the ContractNLI dataset are real contracts collected online. The hypotheses present different assumptions about the content of the contract. This domain is different from the one used for training our models and might present different linguistic characteristics. Therefore, we start by evaluating the NLI performance of our models in a controlled experiment using the oracle spans from the document. 

In Table~\ref{tab:contnli_oracle}, we compare our sentence-pair models, with and without training on ContractNLI, against the SpanNLI model~\citep{koreeda-manning-2021-contractnli-dataset}. SpanNLI was trained with a joint objective for both selecting the evidence spans from the document and making the NLI prediction per hypothesis. The oracle setting disentangles the NLI task from the span selection as the models are provided with the human-selected spans.

Surprisingly, we find our zero-shot sentence-pair NLI models, which were trained on a different domain, outperform the supervised SpanNLI model. \ourmodel , which was trained on all five NLI datasets performs the best, demonstrating strong NLI capabilities. We also train supervised sentence-pair NLI models using the training data from ContractNLI. To collect neutral evidence for training hypotheses with this label, we randomly select a span from the document. As expected, the sentence-pair supervised models outperform the zero-shot models, where the best model is trained over the five NLI datasets in addition to ContractNLI.
Overall, this demonstrates the superiority of the sentence-pair setting over joint objective models.


\subsection{NLI vs.\ similarity-based retrieval}
Given the promising NLI performance of sentence-pair models, we now turn to the task of identifying the relevant evidence per hypothesis in order to devise the full pipeline.
Our retrieval procedure is based on the same sentence-pair NLI models and uses the $p_e$ and $p_c$ scores of each document span against the hypothesis. We argue that if the model can successfully distinguish neutral from informative relations, we can use these scores for both retrieval and classification. Indeed, we find \ourmodel's NLI scores to provide very strong retrieval signal. 
\ourmodel ranks one of the annotated spans as the top-1 span 61\% of the time. A random baseline, in comparison, achieves less than 1\%.
% Compared to a random baseline of less than 1\%, the top-ranked span by \ourmodel's NLI scores is one of the human-annotated spans 61\% of the time.

We also experiment with similarity-based retrievers that rank the spans by the cosine similarity with the hypothesis using TF-IDF vectors~\citep{koreeda-manning-2021-contractnli-dataset}, BERT large embeddings~\citep{devlin-etal-2019-bert}, or SentenceT5 embeddings~\citep{ni2021sentencet5}. Table~\ref{tab:contnli_res} shows the precision at recall 0.8 for these zero-shot retrievers. NLI-based retrieval outperforms the similarity-based methods. Intuitively, this can be explained by the fact that two \emph{neutral} sentences can be very similar according to many measures, but uninformative for our purpose. (e.g., consider $\prem=$``$\textit{We discuss } \hyp \textit{ later}$''). Table~\ref{tab:contract_ret_examples} shows an example of such case.

\subsection{Retrieve-and-classify over documents} \label{sec:ret-and-cls}
We are now equipped to perform both evidence retrieval and classification with the same sentence-pair NLI model. First, we compute the pairwise $p_{y,i}$ scores for $\hyp$ against each span $S_i$. 
We define two methods for constructing the final prediction:
% To construct a final prediction, we define the following two methods:

\paragraph{Retrieve-and-Predict.} We aggregate over all spans by $\bar{p_y} = \max_{i}{(p_{y,i})}$, and then predict by the highest NLI score: 
% \vspace{-.5em}
\begin{equation*}
\begin{small}
\text{prediction} =
\left\{
	\begin{array}{ll}
		\argmax{(\bar{p_e},\bar{p_c})}  & \mbox{if } \max{(\bar{p_e},\bar{p_c})} > T,  \\
		\text{'neutral'} & \mbox{otherwise.}
	\end{array}
\right.
\end{small}
% \vspace{-.5em}
\end{equation*}
We simply set $T=0.5$ for the zero-shot setting, but it can be potentially tuned. Effectively, the prediction is determined by the span with the strongest sentiment towards the hypothesis.

\paragraph{Retrieve-and-Rerank.} For non-neutral predictions, we rerun the same NLI model with the top-K ranked spans retrieved for 'e' and 'c' relations. For symmetry, we do this twice, concatenating the two spans in both orders, and average the scores. Figure~\ref{fig:rerank} illustrates this process with $K=1$.

The reranking method allows the NLI model to directly contrast the span that is most entailing with the span that is most contradicting the hypothesis. 
The resultant multi-sentence premise is longer than \ourmodel's training distribution. Motivated by our earlier findings (\S\ref{sec:docnli_by_len}), we expect the model to generalize to this slightly longer but focused premise.
% This focused comparison creates a short two-sentence premise that is still relatively close to the training distribution of sentence-pair models.

% results with rerank, and compared to SpanNLI
\paragraph{Results.}
Table~\ref{tab:contnli_res} shows the main results on ContractNLI comparing sentence-pair zero-shot models with supervised ones. Surprisingly, the zero-shot sentence-pair models are competitive with the supervised SpanNLI model, even outperforming them in $F_1$(C). The supervised sentence-pair model trained on all five NLI datasets and ContractNLI performs best overall. Its retrieval performance still lacks behind SpanNLI, possibly due to only sampling random spans for neutral examples.
% the random sampling of neutral spans that doesn't utilize the full document.

% The rerank approach provides an average increase of $0.1$ $F_1$ points over the naive aggregation with zero-shot \ourmodel.
Reranking significantly improves the performance of zero-shot \ourmodel, increasing the average score by up to 27\%. We observe better performance with larger context ($K=5$).  For the supervised \ourmodel model, reranking provides only marginal gains, and increasing the context is not beneficial.

% back to DocNLI results
Returning to the DocNLI dataset, we test if our sentence-pair method can improve the low performance over long premises (\S\ref{sec:docnli_by_len}). We focus on examples with a short hypothesis (up to 20 tokens) and long premise (more than 512 tokens). Naively applying \ourmodel on these cases without sentence splitting leads to a low $0.21$ $F_1$ score. Using our retrieve-and-predict approach, the score increases up to $0.41$. Reranking doesn't seem to improve in this case, possibly due to the two-way classification format of that dataset.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/nli_rerank_2.pdf}
      \vspace{-8pt}
    \caption[]{NLI-based retrieve-and-rerank pipeline.}
      \vspace{-5pt}
    \label{fig:rerank}
\end{figure}


\begin{table}[t]
\small
    \centering
        \resizebox{\linewidth}{!}{
    \begin{tabular}{l|c|c|ccc}
    \toprule
    Model & S.P. & P@R.8 & $F_1$(C) & $F_1$(E) & AVG \\
    \midrule
    Majority vote$^{\ddag}$ &  &  - & .083 & .428 & .256 \\
    \midrule
    \multicolumn{3}{l}{\underline{\textit{supervised:}}} \\
        SpanNLI-base$^{\ddag}$ & & .663 & .287 & .765 & .526\\
        SpanNLI-large$^{\ddag}$ & & \textbf{.793} & .357 & \textbf{.834} & .595 \\
        T5-large & v & .575 & .512 & .691 & .601\\ 
        % $\quad$ + rerank & v & - & .519 & .699 \\
        \ourmodel$_{\text{+Cont.NLI}}$ & v & .580 & .521 & .754 & .637\\
        \ + Rerank$_{(K=1)}$ & v  & " & \textbf{.537}  & .741 & \textbf{.639}\\
        \ + Rerank$_{(K=5)}$ & v & " & .520 & .719 & .619 \\
     \midrule
    \multicolumn{3}{l}{\underline{\textit{zero-shot:}}} \\
        TF-IDF$^{\ddag}$ & v & .057 & - & - & -\\
        BERT emb. & v & .083& - & - & - \\
        SentenceT5 & v & .311& - & - & - \\
        T5$_{\text{MNLI}}$ & v & .397 & .261 & .551 & .406 \\
        % $\quad$ + rerank & v & - & .350 & .639 & .494\\
         T5$_{\text{*NLI}}$ & v & .397 & .247 & .594 & .420 \\
        %  $\quad$ + rerank & v & - & .341 & .656 & .499\\
         \ourmodel & v & \textbf{.412} & .257 & .573 & .415 \\ 
         \ + Rerank$_{(K=1)}$ & v & " & .363 & \textbf{.659} & .511 \\
         \ + Rerank$_{(K=5)}$ & v & " & \textbf{.404} & .652 & \textbf{.528} \\
     \bottomrule
    \end{tabular}
    }%
    \vspace{-5pt}
    \caption{Evidence retrieval and classification results of both supervised and zero-shot models on ContractNLI test set. Within sentence-pair (S.P.) models, NLI-based retrieval is more precise than similarity retrievers. Supervised S.P.\ models  outperform the joint SpanNLI model in the final classification task thanks to better $F_1$(C). $^{\ddag}$Results from \citet{koreeda-manning-2021-contractnli-dataset}.}
    \label{tab:contnli_res}
    \vspace{-8pt}
\end{table}

% \subsection{Multi-sentence hypotheses}
% \tal{possibly include SummaC here}

==> sections/long_inputs.tex <==
\section{Long and OOD Inputs}\label{sec:docnli}



\begin{table}[t]
\small
    \centering
    \begin{tabular}{l|cc}
    \toprule
    Model & Dev. & Test \\
    \midrule
    Random & .198 & .199 \\
    \midrule
    \multicolumn{3}{l}{\underline{\textit{supervised:}}} \\
    Longformer-base$^*$~\citep{yin-etal-2021-docnli} & .462 & .444  \\
     Roberta-large~\citep{yin-etal-2021-docnli} & .631 & .613  \\
     T5-large & .642 &.618 \\
     \midrule
    \multicolumn{3}{l}{\underline{\textit{zero-shot:}}} \\
     \ourmodel & .341 & .345 \\     
     \ourmodel$_{\text{tuned}}$ & .409  & .408 \\  
     \bottomrule
    \end{tabular}
                   \vspace{-5pt}
    \caption{$F_1$(E) scores on the \textsc{DocNLI}(-ANLI) binary classification dataset. The zero-shot shot predictions are based on a threshold $T$ on the entailment score which is either set to $0.5$ or \emph{tuned} over $0.2\%$ of the dev set. $^*$Longformer's scores are over the full DocNLI.}
    \label{tab:res_docnli}
    \vspace{-8pt}
\end{table}


We start by exploring the use of \ourmodel on examples that differ from the training data in both length and domain. We hypothesis that a robust semantic reasoning model trained on top of a large LM that memorized world knowledge, should achieve competitive results even when applied to a new domain without any finetuning (i.e., zero-shot). 

For this experimentation, we use the DocNLI dataset~\citep{yin-etal-2021-docnli} and remove ANLI from it since ANLI was included in our training data.\footnote{The ANLI examples cover only 1.2\% of the DocNLI test set, so the difference is minimal. \ourmodel and \ourmodel$_{\text{tuned}}$ get .350 and .410 $F_1$ scores on the full test set, respectively. } 
A large portion of DocNLI is based on news articles where the hypothesis is a short summary of an article and the premise is the article itself. 

DocNLI uses only two classes, ``entail'' vs.\ ``not entail'', by merging the ``neutral'' and ``contradiction'' definitions. We discuss different zero-shot aggregation techniques from 3-way models to binary classification in Appendix~\ref{sec:binary_aggr}.
The ``not entail'' instances are created with both rule-based and LM-based local perturbations techniques over the positive pairs. This results in a slightly different task definition than NLI since in practice even altered (i.e., ``fake'') texts can still factually agree with the hypothesis~\citep{schuster-etal-2020-limitations}. \citet{yin-etal-2021-docnli} account for this discrepancy by augmenting the training set, but zero-shot NLI models might be affected by this provenance-based rather than factual-based partition of the test set.
%


% adapting to 2-way classification





\subsection{Out-of-the-box adoption}
\citet{yin-etal-2021-docnli} found a model with an input limit of 512 tokens to perform well on DocNLI, by simply truncating the remainder of the input.
% , suggesting that the relevant information for prediction mostly appears at the beginning of the premise. 
We follow their setting and evaluate a naive zero-shot application of \ourmodel on this new domain. Table~\ref{tab:res_docnli} shows that \ourmodel performs much better than a random baseline and is competitive with some of the supervised models, indicating promising transfer potential.
% This suggests that \ourmodel is basing its predictions on features that are general enough to transfer to new domains and settings.

\subsection{Performance by input length} \label{sec:docnli_by_len}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.46\textwidth]{figures/docnli_by_length.png}
        \vspace{-4pt}
    \caption[]{Effect of input length of DocNLI examples on naive applications of \ourmodel (zero-shot, without sentence splitting). The blue line shows $F_1$ score as a function of hypothesis length ($|\hyp|$). The orange line bins examples by the premise length ($|\prem|$), focusing only on short hypotheses (where $|\hyp|\le20$). For short hypotheses, the performance stays high even beyond the training distribution, but sharply drops around the input length limit of the model.}
    \label{fig:docnli_by_len}
     \vspace{-5pt}
\end{figure}

Figure~\ref{fig:docnli_by_len} shows the $F_1$ score of \ourmodel as a function of the input length. 
Our first observation is that the performance is highly affected by the length of the hypothesis. \citet{yin-etal-2021-docnli} observed a similar trend even with supervised models. We conjecture that this is due to the natural increase in ambiguity with the hypothesis' length, as it is more likely to contain multiple atomic facts and it's unclear which is the one in question. This motivates our inference pipelines in the following sections that focus on concise hypotheses and aggregate when needed.

Second, we look at the performance as a function of the premise length. To focus on examples where the hypothesis is well defined, we only consider cases with a short hypothesis of no more than 20 tokens (total of 5,932 cases from DocNLI(-ANLI) test set). As the orange line in Figure~\ref{fig:docnli_by_len} shows, \ourmodel performs well on these cases even when the premise is much longer than the inputs that the model was trained on, demonstrating promising potential for zero-shot applications. However, the performance significantly drops when reaching the input length limit, requiring to truncate the premise. Next, we discuss methods for retrieving and aggregating predictions of sentence-pair models over long documents.

% Second, we see that the performance gradually decreases with the total input length, though remains better than random even beyond the model's input limit. This aligns with the earlier observation that in many of the dataset examples the crucial information is at the beginning of the premise. Yet, in some long inputs the model might be missing important information.

% \subsection{Breaking down long premises}
% To address the premise length limitation with a zero-shot NLI model, we split each long premise into multiple sentences, evaluate the hypothesis against each of them independently, and aggregate the scores by taking the max $p_y$ across sentences. To evaluate this approach, we collect examples with a short hypothesis ($<20$ tokens) and long premise (combined length over 512 tokens) from the test set. Without splitting, \ourmodel's $F_1$ score on this subset is only $0.228$, only slightly above random.

% Following the splitting and aggregation approach, predicting with 'c' threshold achieves $0.333$ $F_1$ with $T=0.5$, and up to $0.412$ with $T=0.2$. In this setting, 'e' threshold reaches only $0.239$ $F_1$.

% more expensive but can be run in parallel, unlike models that process very long inputs and have to run self-attention on long input.

% Instead, we aggregate the predictions per hypothesis by taking the maximum $p_y$ across all predictions against each of the premise sentences.

